Democratizing Reward Design for Personal and Representative Value-Alignment

Aligning AI agents with human values is challenging due to diverse and subjective notions of values. Standard alignment methods often aggregate crowd feedback, which can result in the suppression of unique or minority preferences. We introduce Interactive-Reflective Dialogue Alignment, a method that iteratively engages users in reflecting on and specifying their subjective value definitions. This system learns individual value definitions through language-model-based preference elicitation and constructs personalized reward models that can be used to align AI behaviour. We evaluated our system through two studies with 30 participants, one focusing on "respect" and the other on ethical decision-making in autonomous vehicles. Our findings demonstrate diverse definitions of value-aligned behaviour and show that our system can accurately capture each person's unique understanding. This approach enables personalized alignment and can inform more representative and interpretable collective alignment strategies.

==> versions/v1.apr.2/1_introduction.tex <==
\section{Introduction}
\carter{Emphasize the relationship between alignment and reward modelling?}

% \subsection{What are we trying to do and why is it relevant?}
How should AI agents act? There is no single universally satisfying answer to this question, as people have diverse preferences and values that are shaped by their personal backgrounds. 

Recently, reinforcement learning from human feedback (RLHF) has emerged as a popular and effective method for aligning AI systems to human goals and desires~\cite{casper_open_nodate}, but the feedback generally used in this process is aggregated over many individuals \cite{bai_training_2022}. In aggregating feedback, personal differences in beliefs about how an agent should act are "averaged" out, which can lead to systems that ignore the preferences of minority groups or those with uncommon or unique preferences~\cite{siththaranjan2023distributional}.

As AI systems and agents enter more sensitive and personal parts of our lives, such as our homes, we should be conscious of what values they possess and who decides what they are. Take, for example, the desire for respectful interaction from an AI agent within a household. The agent's behaviour should align with the unique interpretation of respect held by the individual or family using it, as another person's conception of respect might vary widely based on their background. While this may seem obvious, as mentioned above, AI systems are usually either aligned to an aggregated group definition of a value or behaviour (through large-scale human-feedback data collection) or to the system designer's definition of desirable behaviour (as in traditional RL). 

Since values and preferences are personal, there is a need for an accessible way for end users of AI systems to train agents to embody their individual definition of desirable behaviour. This requires an accessible way for users of AI systems to express their desires and goals to the system and an effective way to model these desires and goals so that they can be incorporated and embedded into AI systems and agents.


% It has been acknowledged in the AI community that the best method for humans to interact with the system to express their goals and desires is still an open problem in human-computer interaction\cite{casper_open_nodate}. The solution for doing this needs to be accessible, as people without expertise in machine learning may wish to use AI systems to their desires. For example, imagine a person who purchases a humanoid robot to do household chores and wants the robot to act respectfully in their home according to their definition of respect. As part of being accessible, the system must be sample-efficient and minimally time-consuming, as people may not have days of free time to teach an AI system how to act appropriately. And the system must accurately capture the given individuals' desires and preferences.

% \subsection{Why is it hard?}

The exact way to align an AI agent's behaviour to human goals and desires is currently an open and difficult problem. Reinforcement learning from human feedback (RLHF) is a promising method, but it has been acknowledged in the AI community that the best method for humans to interact with the system to express their goals and desires is still an open problem in human-computer interaction~\cite{casper_open_nodate}. When narrowing the problem down to aligning an agent to a single individual's preferences, the problem becomes even more difficult. This is because we must consider that individual users may not have a technical background or the time necessary to undergo rigorous training on how to give feedback to an agent~\cite{bai_training_2022}. Further, individuals may not have the time to spend days teaching a data-hungry agent how to behave. As such, a system that allows end users to align agents to their unique individual values should have the following properties:
\begin{enumerate}
    \item The system should be accessible to users of all backgrounds and not require any special technical knowledge.
    \item The system should be sample-efficient and minimally time-consuming for the user.
    \item The system should be able to capture individual differences and unique conceptions of desirable behaviour.
\end{enumerate}

Each of the aforementioned properties places constraints on the development of a system for aligning agents to individual desires, making an already unsolved problem more difficult. For example, it is common for those giving feedback to agents to undergo rigorous training on how to do the labelling~\cite{bai_training_2022}, but in our case, this is not feasible as it limits accessibility and usability. Further, it is common to collect hundreds \cite{christiano_deep_2017} or even hundreds of thousands of labelled examples~\cite{bai_training_2022} for RLHF, but in our case, we need to suffice with only a handful of examples to respect users time. 

% \subsection{How do we solve it?}
As a step towards successfully aligning AI agents to individual preferences, we present \systemname{}. The user-facing side of our system is a simple chat interface where the system prompts the user to explain the behavioural pattern they would like the agent to embody. The system sends textual messages and videos of the agent behaving and collects language feedback from the user. We choose the videos to collect feedback on using techniques from active learning, an area of human-in-the-loop machine learning \cite{mosqueira-rey_human---loop_2023}. In particular, we use diversity-based sampling to find videos where the agent is behaving in varied and diverse ways to elicit a wide range of information from the user. We also rely on uncertainty-based sampling to find videos where the system is unsure how the user would like the agent to act. The system's textual messages are designed to make the user reflect and think deeply about their preferences and values and is inspired by work done on designing for reflection \cite{fleck2010reflecting, wolfbauer_script_2022, kocielnik_reflection_2018, bentvelzen_revisiting_2022}. Using the information gained from the dialogue-based preference elicitation, we create a language-based reward model that relies on the in-context learning abilities of large language models~\cite{brown_language_2020}. 

% \subsection{How do we verify we solved it?}
We evaluated \systemname{} with a 21-user study where participants used the system to build a reward model for their own personal definitions of respectful behaviour. We found that the reward model generated by our system aligns more closely with an individual user's actual reward model than the alignment observed among different participants. This suggests that our system can more accurately predict a user's perception of an agent's respectful behaviour compared to predictions made by another individual using their own understanding of respect.

We also compare our system to a baseline inspired by \cite{kwon2022reward}, where only explained examples are used to generate a reward model on the user's behalf. We show that our system significantly outperforms the baseline in capturing individual human preferences. 

% \subsection{Contributions}
Our contributions are as follows:
\begin{itemize}
    \item A novel, accessible and theoretically justified pipeline for aligning AI agents to individual values and preferences that draws upon insights from a wide range of AI, HCI, and social science research
    \item An evaluation of the system that demonstrates its ability to capture individual human preferences and values
    \item The introduction of an important and understudied question in HCI: How to best collect human feedback for RLHF
    \item \carter{Maybe mention that we are the first to extend language reward to non-text environments?}
\end{itemize}

Our system does not solve the problem of individual value alignment but takes a step towards a solution. We hope this work inspires other HCI researchers to work on this difficult problem.

% \carter{Old below}
% Hook argument: Values are personal and subjective. Different people will have different ideas about what is respectful or appropriate. As such, if we train monolithic systems that try to satisfy everyone, we will end up disappointing some people. The current approach to aligning large AI systems to human values aggregates over many people and aligns to the majority. If robots or AI systems are in the home, then people will want the agent aligned to their own definition of what is respectful, not an average definition or the definition of some system designer. People need an accessible lever to shape the behaviour of agents to their liking and personalize them to align with their own definitions of values. Reinforcement learning is a common approach to training agents. We can use rewards to shape the behaviour of agents, but a person cannot sit around all day, labelling examples of acceptable behaviour. Our system must be accessible, sample efficient (low effort), scaleable, and accurate capture the users personal subjective definition of a desireable behaviour pattern or value. 

% Human preferences and values are diverse among different people. 

% \carter{Old below}

% Human social values can help guide \textit{human} decision-making to favourable outcomes \cite{ravlin1987effect}. However, we are offloading ever more of our decisions to artificial intelligence (AI). As such, we may want AI agents to embody the same desirable social values as humans do. Ravlin and Meglino define social values as "general modes of behaviour that an individual 'should' or 'ought' to exhibit. In short, we can think of social values as complex behaviours or behavioural patterns that are favourable to society. For example, we may want the AI agents we train to be respectful or embody environmental behaviour.

% However, historically, it has been found to be difficult to get AI agents to reliably embody even well-defined and relatively simple behavioural patterns (amodei and olah, 2016). In reinforcement learning, the main approach used to train AI agents that will continuously interact and learn from an environment, the designer of the agent must come up with a reward function that defines desirable behaviour and rewards the learning agent accordingly. If the designer fails to align the reward signal to the desired behaviour, "reward hacking" can occur where the agent learns some behaviour that receives a high reward but which betrays the designer's intent. As a simple example, imagine that the designer of a floor-cleaning robot gives the robot a reward for sweeping up dirt. On the surface, this does not seem like a bad reward signal since sweeping up dirt should make the floor cleaner. However, the agent may learn to throw copious amounts of dirt on the floor in order to clean it up and receive a reward. Underspecified reward function is the cause. 

% While designing rewards for simple and well-defined behaviours like cleaning the floor can be difficult, the problem of reward design only becomes more difficult as the desired behaviour becomes more abstract. Human values are abstract, and different people may have different definitions of certain values. This makes designing reward functions that reliably incentivize value-aligned behaviour even more difficult. 

% Traditional function-based reward functions may have a difficult time capturing values, as values can be defined as a behavioural pattern, not an atomic action or state. This violates the Markov property, so value driven reward may need to be non-Markovian (Wirth Survey, 2017). Further, traditional function-based reward function design is extremely inaccessible, and the task is usually only undertaken by a single individual or a small group of individuals. This is because traditional reward design is difficult to do an is often thought of as more of an art than a science. This is generally undesirable as it means a small number of people get to choose how an agent that could interact with many people will behave. Lastly, traditional reward functions are notably inflexible, which can make them more susceptible to reward-hacking.

% More modern model-based approaches to reward design use machine learning to learn a reward model. This allows for a more nuanced and flexible reward function as the function is learned as opposed to hard-coded. Two common approaches are inverse reinforcement learning (IRL) and reinforcement learning from human feedback (RLHF). In IRL, the reward model is learned from expert (usually) human demonstrations. The goal is to infer what reward function the agent in the demonstrations is following, assuming the actions taken in the demonstration are optimal with respect to the hidden reward function. This approach can be effective but usually requires thousands of demonstrations. Further, IRL usually learns from a pool of trajectories and cannot obtain new feedback in the face of uncertainty (Wirth Survey, 2017).  In RLHF, human feedback on the actions of an agent is elicited, then the feedback and action data are used to learn a model of which actions a human finds desirable. Generally, both approaches require many, many samples to learn the reward model, which can be expensive or, in some cases, infeasible. Even for simple tasks, RLHF can require 700 user-labeled examples (Christiano et al., 2017), and for more complex tasks, this approach can require hundreds of thousands of human-annotated examples (Bai et al., 2022). Both of these approaches assume the humans being learned from have a perfect understanding of their own preferences which is not always the case (NEED GOOD FOUNDATIONAL CITATION FROM PREFERENCE ELICITATION LIT)

% RLHF in particular is the most popular approach to align agents with human values. A recent survey on the topic noted that many of the open questions in regard to RLHF have to do with human-computer interaction.  In particular they note, "Specifically, it is unclear what type of feedback (or combination thereof) is optimal for learning human goals, precisely how biases harm the quality of feedback, and how to best select and train human evaluators. As discussed in Section 3, human desires are difficult to express with a reward function (Skalse and Abate, 2022b; Bowling et al., 2023; Vamplew et al., 2022)" They also note that "An individual human’s values are difficult to represent with a reward function." They also note that "Using language, humans can convey a large amount of information per evaluation, reducing ambiguity and goal misspecification." They also note that ". However, AI-generated feedback has drawbacks. Humans often disagree with AI feedback. The rate of human/AI disagreement will vary by task, but Perez et al. (2022b), Casper et al. (2023b), and Lee et al. (2023) found this to happen up to 10\%, 46\%, and 22\% of the time respectively in different experiments."

% RLHF creates a massive joint reward model which requires many many data points and averages over individuals in undesirable ways. Traditional RLHF cannot be personalized because it requires so many data points. this means that some users can get averaged over in undesireable ways (DPL). \carter{Should differentiate between RLHF in general and RLHF for language models}

% If we want to make it personalized, it must be accessible. 

% In order to make reward design more accessible and more able to capture individual human values, we developed a language-based pipeline for reward design that doesn't require the designer to possess any special knowledge. Our approach allows for \textit{anyone} to train an agent to embody a value like respect.

% We leverage reflective techniques from HCI to allow users to better understand their own preferences and values. (to increase accuracy and decrease bias). In particular, we base the reflection on the levels of reflection proposed in \cite{fleck2010reflecting}. Level 1 reflection is defined as a reflective description where the
% Reflection has been found to reduce bias (cite bias), and increase accuracy (cite medical papers). 

% We leverage dialogue-based preference elicitation to capture information about the user's preferences that can be used for a language-based reward model. We couple reflection with both item-based and feature-based preference elicitation to better understand users' preferences (Priyogi, 2019).

% We use active learning with both diversity-based and uncertainty-based sampling to select good items (trajectories) for the user to label (Mosqueira-Rey et al., 2023)

% We leverage the textual preference information from the dialogue-based preference elicitation and LLM's in-context learning ability (Language Models are Few-Shot Learners, 2020) to develop a language-based reward model.

% We employ multiple feedback loops to allow for iterative reflection and refinement

% Lastly, we have an interactive approach which leverages interleaved preference query generation (Wirth Survey, 2017)

% Most other language-based reward systems are computationally inefficient due to the size of LLMs and the expense of querying them. In order to overcome with we leverage the reward model built with RLHF to train an SL (RNN) reward function using RLAIF.  Talk about improved efficiency and scalable oversight. (hierarchy of scalable oversight: human < llm < rnn)

% Value sensitive design

% from "Fundamental issues with RLHF paper":
% \begin{itemize}
%     \item three main parts of RLHF: "preference elicitation, fitting a reward model, and policy optimization" (p 18)
%     \begin{itemize}
%         \item We focus only on preference elicitation and fitting a reward model.
%     \end{itemize}
% \end{itemize}

% Talk about how LLM reward function are expensive and thus are not scalable. (SCALABLE SUPERVISION IS IMPORTANT - concrete problems in AI safety. Amodei and Olah et al.)

% Contributions:
% \begin{itemize}
%     \item a pipeline for integrating values into an AI agent
%     \item (weak)?? Environment for value learning?
%     \item (weak)?? Evaluation of inter-labeler disagreement on values
%     \item (weak)?? Connecting VSD, Reflection, DBPE, AL, IML, ICLBRM, (I)-RLHF opening the door to new fruitful collaborations and interdisciplinary research.
%     \item We are the first to use a combination of script-based dialogue and LLM text for reflection.
% \end{itemize}
% \section{Related Work}
% Value alignment

==> versions/v1.apr.2/2_background.tex <==
\section{Background and Related Work}
Our work falls at the intersection of human-computer interaction and reinforcement learning. We drew on insights from AI, HCI, and social science research in developing our system to accurately capture individual preferences in a reward model. Below we outline the related work most relevant to our system and give the necessary background to understand it.

\subsection{RL, Inverse RL \& RLHF}
In reinforcement learning (RL) an agent learns how to act in an environment to maximize the rewards it receives. Traditionally, the agent designer designs a reward function that is intended to incentivize desireable behaviour, as defined by the designer. However, reward design is notoriously challenging and can result in reward hacking where an agent learns behaviour that gets high reward, but that betrays the designers intent \cite{amodei_concrete_2016, dewey2014reinforcement, everitt2016avoiding}.

In response to difficulties with reward design, inverse reinforcement learning (IRL) was developed. In IRL the goal is to \textit{learn} a reward function from expert demonstrations \cite{ng2000algorithms, ramachandran2007bayesian, abbeel2004apprenticeship, ziebart2008maximum, neu2009training}. This can be useful when a desired behaviour is easy to demonstrate but difficult to design a reward function for. However, since multiple reward functions can often explain the observed behaviour of the experts, the reward function lacks interpretability and is inherently ambiguous \cite{metelli2023towards}. Recently, Kwon et al. \cite{kwon2022reward} proposed a pipeline that relies on large language models in-context learning ability to learn a reward function from a small number of demonstrations, albeit accompanied by explanations, in text based environments. 

Reinforcement learning from human feedback (RLHF) instead learns a reward model from human feedback \cite{christiano_deep_2017, ziegler2019fine, bai_training_2022} as opposed to expert demonstrations. This approach is especially when attempting to align agents to human preferences as the agent can optimize for getting \textit{good} feedback. There are three main parts of RLHF: Feedback collection where humans provide feedback, reward modelling where the feedback is turned into a reward model, and policy optimization where the reward model is used to train a policy/agent with reinforcement learning \cite{casper_open_nodate}. The most common RLHF methodology uses binary preference data obtained through pairwise comparison feedback \cite{christiano_deep_2017}, however more recently language feedback has been used as well \cite{bai_constitutional_2022, kwon2022reward, scheurer2022training, chen2023improving}.

% RLAIF

\subsection{Dialogue-Based Preference Elicitation}

When using language feedback for RLHF it is natural to frame the feedback collection as dialogue-based preference elicitation. In dialogue-based preference elicitation, the goal is to understand a users preferences through the use of dialogue \cite{priyogi_preference_2019, radlinski_coached_2019}. In preference elicitation there are two main approaches, each with their own benefits and drawbacks; item-based preference elicitation where the user is asked about their preferences about specific things \cite{adomavicius2005toward, sarwar2001item, loepp2014choice, christakopoulou2016towards, graus2015improving} and feature-based preference elicitation \cite{llorente2011increasing, sun2018conversational, viappiani2006preference}. Some methods use both item- and feature-based methods \cite{biyik2023preference}, similar to our approach. Recently large language models have been used for dialogue based preference elicitation as well \cite{li2023eliciting, verma2023preference, jeong2023factual}.


\subsection{Active Learning}
When performing preference elicitation, in particular item-based preference elicitation, we must select items to query the user about. Active learning is a subfield of machine learning where the learner is responsible for choosing which examples to request labels for \cite{settles2009active, ren2021survey}. Being selective about which examples to query the user about is important in cases where labels are expensive to obtain \cite{olsson2009literature}. For example, in our case we must ask the user to label and explain each trajectory they see which is time consuming for the user.

There are generally three strategies for sampling items to query the user about, namely random-, diversity-, and uncertainty-based sampling \cite{monarch2021human}. Random-based sampling randomly selects items to query the user about, diversity-based sampling aims to select samples that are different from one another to get information about more parts of the input space, and uncertainty-based sampling seeks to select items that the model has low confidence about.

\subsection{Reflection}
Designing for reflection has been of interest to many HCI researchers for some time \cite{price2003new, yukawa2003co, rogers2006framework, lindstrom2006affective, ghajargar2018designing}. However, Fleck \& Fitzpatrick note that ``designing for reflection'' can mean different things to different researchers~\cite{fleck2010reflecting}. Accordingly, they propose a framework that can be used to think about designing for reflection. Their ``levels of reflection'' and ``techniques for supporting reflection'' are of particular importance to our work. They define level zero of reflection as just revisiting past events. Level one is defined as revisiting with explanation where the one reflecting explains and rationalizes events. Level two of reflection is defined as dialgoic reflection where relationships in the information and differing perspectives are considered. Level three reflection is transformative where the reflection prompts a change in ones actions. And level four of reflection is critical reflection  which involves taking into consideration wider contexts such as social or moral considerations. 

Previous work has used language prompts to engage users in reflection~\cite{fessl2017known, renner2016effects, williams2016revising, ifenthaler2012determining}, where single questions or sentence starters are offered to the user. Other work has extended this to use scripted multi-message dialogue to guide users through reflection  \cite{kocielnik2018reflection, wolfbauer2022script}.

The recent rise of LLMs and their chat interfaces presents the opportunity for more tailored and dynamic dialogue to engage users in reflection, however, there has been relatively little work exploring this. Some work has explored the use of LLMs for generating reflective prompts in a design template~\cite{yin_jamplate_2024}. However, to the best of our knowledge, there has been no work, aside from ours, on integrating LLMs into reflective, back-and-forth dialogue with a user.

Reflection also has several notable benefits. For example, it has been found that prompting medical practitioners to engage in reflection can increase diagnostic accuracy~\cite{costa2019effects, fernandes2021adding, mamede2008effects}. And, more relevant to this work, in consumer research, it has been found that prompting consumers to engage in preference self-reflection can lead to more accurate reporting of preferences~\cite{hauser2014self}. Further, it has been found that engaging consumers in realistic decisions can increase preference elicitation accuracy \cite{hauser2014self}. As our system is concerned with gaining an accurate account of user's preferences and intent, these findings are of particular relevance.

==> versions/v1.apr.2/3_system.tex <==
\section{System}
The three main parts of reinforcement learning from human feedback are \textbf{feedback collection}, \textbf{reward modeling}, and policy optimization \cite{casper_open_nodate}. Our system, \systemname{}, focuses on feedback collection (subsection \ref{feedback_collection}) and reward modeling (subsection \ref{reward_modeling}), and is compatible with nearly all policy optimization methods.

\systemname{} allows users with no particular expertise in machine learning to generate a reward function that can be used to train agents that embody individually value-aligned behaviours. The user-facing side of the system is a simple chat interface where the user converses with the system. On the backend, we use the information collected during the conversation with the user to create a reward model that captures the preferences of the user. The reward model generated by the user can then be used to train an agent. If the behaviour of the trained agent is not satisfactory to the user, the system could collect additional information from the user about the behaviour of the trained agent to refine the reward model. This process could cycle indefinitely between feedback collection and reward modelling with \systemname{} and policy optimization until the user is satisfied with the behaviour of the agent.

We will begin by providing a high-level overview of the system and then describe each component in more detail.

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/RLHF_pipeline.png}
  \caption{\todo{Placeholder image for now }Overview of RLHF pipeline with \systemname{}}
  \Description{}
\end{figure}


\subsection{System Overview}
This system overview is described here in words and more briefly in \todo{ALGORITHM 1}.

To begin, we allow the user to specify how they would like the agent to act in natural language. For example, a user could say something as simple as ``I would like the agent to act respectfully.'' We assume the agent has not been trained, so we collect a large pool of trajectories (sequences of the agent taking actions in the environment). We then use \textit{diversity-based trajectory sampling}, a technique from active learning, to find $k$ trajectories where the agent behaves in diverse ways. The goal of diversity-based sampling in this case is to find trajectories where the agent acts according to the users instruction and where it does not. The system then shows the user these $k$ trajectories one at a time and asks the user to explain if the agent is acting according to their instruction.

Based on the way the user responds to each trajectory, the system makes a hypothesis regarding the behavioural features on which the user bases their decisions. The system also proposes additional features that could be relevant to the user. The user is then prompted to reflect on whether the hypothesis is correct and why or why not the additional features proposed are relevant to their desired agent behaviour. If the user agrees with one of the additional features proposed by the system, or has changed their mind in another way as a result of this reflective step, they can enter into the \textit{preference clarification loop} and re-explain the $k$ trajectories they initially saw with their new perspective.

All of the information collected from the user is then used to make a temporary language-based reward model. This temporary reward model is then used for \textit{uncertainty-based trajectory sampling}. The temporary reward model assigns binary rewards (0 if the user would not approve of the agents behaviour and 1 if the user would approve of the agents behaviour) to a small pool of trajectories. The trajectory where the model is least certain about the reward to assign is then shown to the user and they are asked to explain why or why not the agent behaves as they would like it to. A minimum certainty threshold can be set and this uncertainty reduction process can be repeated until the model is at least as certain as the threshold about every trajectory in the uncertainty pool. Each time the user explains one of the trajectories the model is uncertain about, this information is added to the reward model, thus making it less uncertain about similar trajectories.

Ultimately, all of the information gained from the user is combined into a language-based reward model that can effectively administer rewards to the agent when it acts in accordance with the way the user would like it to. This reward model can then be used to either train a more efficient reward model or to train an agent directly depending on the complexity of the desired behaviour and environment. 

\subsection{Feedback Collection} \label{feedback_collection}
In the spirit of making our system accessible to users with varying backgrounds and skill sets, we collect feedback from users in natural language through a chat interface. In addition to being a common and accessible mode of interaction, dialogue has been found to be engaging~\cite{ruan2019quizbot, wolfbauer_script_2022}, which makes it an appealing method for feedback collection. We frame our language-based feedback collection as \textit{dialogue-based preference elicitation}, where we collect feedback about users' preferences regarding the agent's behaviour.

\subsubsection{Dialogue-Based Preference Elicitation}\label{dialogue-based_preference_elicitation}

The dialogue-based preference elicitation process is visualized in figure \ref{fig:teaser} and described here in words. 

There are two main approaches to dialogue-based preference elicitation: item-based preference elicitation and feature-based preference elicitation~\cite{priyogi_preference_2019, biyik_preference_2023}. In item-based preference elicitation, users are asked about their preferences regarding particular items or examples. For example, the user could be asked whether an agent acts according to their desire in a particular trajectory. In feature-based preference elicitation, users are asked about their preferences for certain features or attributes. For example, the user could be asked if they approve of some behavioural feature like an agent moving out of the way for a human. Our system employs both item- and feature-based preference elicitation during the dialogue with the user.

\begin{figure}
    \centering
    \begin{lstlisting}
----- Step: 0 -----
The main agent (M) is in the 
quadrant (orchard) that it owns.
 M   .   . | .   G   .
 A   .   . | G   .   .
 .   .   . | .  AA   B
-----------------------
 .   .   . | .   .   .
 B   .   A | B   .   .
 A   .   . | A   A   .

=========================
----- Step: 1 -----
Main agent moved from [0, 0] to [1, 0]. 
 .   M   . | .   G   .
 A   .   . | G   .   .
 .   .   . | .  AA   B
-----------------------
 .   .   . | .   .   .
 B   .   A | B   .   .
 A   .   . | A   A   .
\end{lstlisting}
    \caption{ASCII Encoding of the First Two Steps of Trajectory of a Grid-World Environment Used in Our System Evaluation}
    \label{fig:ascii-encoding}
\end{figure}

\textit{\textbf{Stage 1: Initial Item-Based Preference Elicitation: }}In order to perform item-based preference elicitation, we must first select items to query the user about. For this task, we use techniques from active learning. At the start of the interaction with the user, we lack information about the user's preferences, and thus, we employ \textit{diversity-based sampling} to find a set of trajectories where the agent exhibits a diverse set of behaviours in varying situations. To do this, we begin by sampling a large pool of over 1000 trajectories. We turn each trajectory into a numerical array that gives a full representation of the state of the environment at each time step. For example, in a grid world environment for a 30-step trajectory, we can encode each step as multiple arrays of the same shape as the grid. In each array, for a step, we can encode the position of a certain type of entity within the environment. For example, one of the arrays might contain 1s in each index where an agent resides, and another one of the arrays might contain 1s in each index where apples are located. We can then combine all the arrays from each step into a multi-dimensional array that fully represents the trajectory. 

With the pool of encoded trajectories in hand, we perform $k$-means clustering of the trajectories. This splits the pool of trajectories into $k$ different groups of trajectories where the trajectories in a given group are all similar, but the trajectories from different groups are different. Since we want to query the user about a diverse set of trajectories in this initial phase, we select one trajectory from each of the $k$ groups. In particular, for each group, we select the trajectory closest to the arithmetic mean, or the centroid, of all the trajectories in the group. The goal of this clustering is to find $k$ trajectories to query the user about that are representative of different and diverse types of behaviour.

The system asks the user to explain why or why not the agent is aligned with their preferences in each of the $k$ trajectories one at a time. The system asks the user to explain their reasoning in 1-3 sentences. For instance, if a user were trying to get an agent to behave respectfully, the system would ask, ``\texttt{Does the agent act respectfully? Please explain your reasoning using 1-3 sentences.}''

\textit{\textbf{Stage 2: Feature-Based Preference Elicitation: }}
% \carter{Possibly explain trajectory encoding here?}
Once we have collected information from the user about each of the $k$ trajectories selected through diversity-based sampling, we use a large language model (GPT-4 Turbo) to make a hypothesis about what features the user is basing their decisions on and other features the user could consider. To do so, we parse each trajectory into an ASCII representation (see figure \ref{fig:ascii-encoding} for an example) and pass this to the LLM along with the user's explanation. In the prompt, we ask the LLM to make a hypothesis about what features the user is basing their decisions on and to offer alternative features the user could consider.

For example, in the environment used in our evaluation, where an agent owns one of four orchards in the environment, the user may base their definition of ``respectful'' behaviour on whether the agent stays in its own orchard. A simplified example of a response from the system could be something like:
\begin{quote}
    \texttt{Based on your explanations, it seems as though a key factor in determining whether the agent's behaviour is respectful or not is whether the agent stays in its own orchard.}
    \texttt{You could also consider:}
    \texttt{
    \begin{enumerate}
        \item Whether the agent helps pick up garbage
        \item Whether the agent steals apples from other agents
    \end{enumerate}
    }
\end{quote}

The user is then prompted to explain if the hypothesis the system made is correct and if the other features should be considered. This step is important for a number of reasons. First, understanding the features on which the user bases their decisions allows for improved generalization of the reward model. This is because the system can use these features, or patterns of behaviour, as decision criteria when assessing whether the agent's behaviour in a trajectory aligns with the user's intent. Second, this step encourages the user to reflect on their definition and consider alternative perspectives. This reflection can assist users in gaining a clearer understanding of the specific behaviour they want the agent to demonstrate. Third, if the diversity-based sampling in the initial item-based preference elicitation phase does not select any trajectories where a certain behavioural feature is present that would be important to the user, the alternative or additional features proposed by the system can help uncover these. This can help the system gain a more holistic understanding of the user's preferences, even when only querying the user about a handful of items.

If the user updates the features they think are important based on the system's proposed alternatives, they can optionally re-explain the initial $k$ trajectories. We refer to this as the \textit{preference clarification loop} as it allows users to iteratively reflect on what features or behavioural patterns they would like the agent to embody. This loop simultaneously helps the user better understand their own preferences, and helps the system gain a clearer understanding of the user's true intent. 


\textit{\textbf{Stage 3: Uncertainty-Reduction Item-Based Preference Elicitation: }}Once the user has exited the preference clarification loop, the system creates a \textit{temporary} reward model based on the user's expressed intent. The reward model can be thought of as a classifier - the input is an ASCII representation of a trajectory, and the output should be a 1 if the agent's behaviour aligns with the user's expressed intent and 0 otherwise. The reward model will be covered in more detail in section \ref{reward_modeling}. The reward model is then used to assign rewards to a pool of trajectories. Since our reward model is based on an autoregressive transformer (LLM), we can find trajectories where the reward model had high uncertainty about what the reward should be by comparing the token probabilities for a positive classification (reward) or a negative classification (no reward). For example, if the user is training the agent to be respectful, we compare the probability of the reward model outputting the "respectful" token to the probability of the model outputting the "disrespectful" token. If the probabilities are close to one another, then the model is less certain, and if they are very different (e.g. 0.99 and 0.01), then the model has high certainty about whether the agent acts according to the user's intent. The "confidence" of the model can be thought of as the absolute value of the difference between the two tokens. We can then collect feedback from the user about the trajectory where the model had the lowest confidence. This is an active learning technique known as \textit{uncertainty-based sampling}. Each time we query the user to explain a trajectory for which the model had low certainty, we add the ASCII representation of the trajectory and the user's explanation to the reward model to increase its confidence in similar situations. We can set a minimum confidence threshold and continue to do this until the model's confidence about each trajectory in the uncertainty pool is above the threshold. This is referred to as the \textit{uncertainty reduction loop} as it iteratively reduces the model's certainty about the user's intent.
  
\subsubsection{Reflective Dialogue}
In decision theory, it is acknowledged that many aspects of decision-making can be "fuzzy" \cite{bellman1970decision, ribeiro1996fuzzy}. Ribeiro \cite{ribeiro1996fuzzy} identifies four aspects involved in decision-making. 
\begin{enumerate}
    \item Alternatives: What one is choosing between.
    \item Attributes: The characteristics defining each alternative
    \item Objectives: A set of attributes defined by the decision maker to be the goal
    \item Preferences/weights: The relative importance of attributes
\end{enumerate}
Ribeiro \cite{ribeiro1996fuzzy} notes that the attributes, preferences, and objectives can all be fuzzy. In our case, when the user is deciding whether the agent is aligned with their intent or not, the \textbf{alternatives} are whether or not the agent is aligned with their intent, the \textbf{attributes} are the behaviours of the agent, the \textbf{objective} is for the user to assess if the agent is aligned with their intent based on key attributes, and the \textbf{preferences} are how important the user thinks each behavioural feature or attribute is. 

When determining if the agent is aligned with their intent, the user may not know apriori what behaviours or behavioural features they think are aligned with their intent. They may also not know what behaviours they find most important in determining their stance on the agent's behaviour. This is important as, over the course of a trajectory, the agent might do some things they approve of and other things they don't. Deciding whether the agent is aligned with their intent and to what degree can be a "fuzzy" decision for the user.

To help the user clarify this decision and convey a clearer picture to the system, we designed our dialogue to engage the user in reflective, system 2 thinking \cite{evans2019reflections}. Work on dual process theory has found that intuitive (system 1) and reflective (system 2) thinking may not be completely distinct and, rather, that both systems may cooperate in reasoning and moral reasoning \cite{evans2019reflections, cecchini2021dual}. In particular, it has recently been proposed that reflective system 2 thinking can help one justify, rationalize and explain their intuitions. This insight is extremely important for dialogue-based preference elicitation. \textbf{A user may have an intuitive, fuzzy understanding of how they want the agent to act, but in order for the system to capture this, the user must be able to clearly explain and justify this.} As such, we draw upon insights from HCI research on "designing for reflection"~\cite{fleck2010reflecting} to help the user reflect on and explain their intent to the system.

In particular, we draw on Fleck and Fitzpatrick's levels of reflection and implement techniques they suggest can support reflection, such as asking reflective questions and providing alternative perspectives~\cite{fleck2010reflecting}.

During both stages of item-based preference elicitation (see stage 1 \& stage 3 in \ref{dialogue-based_preference_elicitation}), we designed the system dialogue to engage the user in level 1 reflection, referred to as ``reflective description.'' The system asks the user to state whether the agent acts in the way they desire and to justify and explain their decision. This allows the user to reflect on the reasoning behind their decision and also gives the system more information about the user's intent and preferences. When the user provides a decision and an explanation, the explanation can help the reward model generalize to other situations as it elucidates the features the user is using to make their decisions\cite{lampinen-etal-2022-language, kwon2022reward}.

During the feature-based preference elicitation stage (see stage 2 in \ref{dialogue-based_preference_elicitation}), the system engages the user in level 2 reflection, referred to by Fleck and Fitzpatrick as ``dialogic reflection'' which ``primarily involves seeing things from a different perspective'' \cite[p.~218]{fleck2010reflecting}. To achieve this, we prompt an LLM to make a hypothesis about what features the user is basing their decisions on and to propose alternative features the user could consider. This is then shown to the user, and they are prompted to explain if the hypothesis is correct and why or why not the other features should be considered. Again, in doing this, the user clarifies their own understanding of the behaviour they would like the agent to embody and communicates this to the system.

Overall, the goal of the reflective dialogue is twofold. First, it helps the user clarify their own, possibly fuzzy, preferences. And second, it helps the system understand the user's preferences and intent. 


% Moon describes reflection as ``a form of mental processing with a purpose and/or an anticipated outcome that is applied to relatively complicated or unstructured ideas for which there is not an obvious solution''~\cite[p.~98]{moon_reflection_2000}. 





% \carter{Old below}
% In preference literature, it is known that people may not have a perfectly clear understanding of their own preferences. This is referred to as "fuzzy preferences." \cite{bellman1970decision, ribeiro1996fuzzy}

% Moon describes reflection to be...

% Reflection has been found to increase accuracy in medical diagnosis and reduce bias.

% To incorporate reflection into our system, we draw on Fleck and Fitzpatrick


% The dialogue produced by the system is partially scripted and partially generated by large language models. Since users may not immediately have a clear picture of what the desired behaviour actually looks like in a given environment, we draw on work about designing for reflection~\cite{fleck2010reflecting}. In particular, we design the dialogue produced by the system to prompt the user to engage in various levels of reflection as defined by Fleck and Fitzpatrick \cite{fleck2010reflecting}. During item-based preference elicitation, we prompt the user to engage in level-1 reflection, referred to as reflective description,  which is defined as "description including justification or reasons for action or interpretation, but in a reportive or descriptive way." During feature-based preference elicitation, we prompt the user to engage in level-2 reflection, defined as "Looking for relationships between pieces of experience or knowledge, evidence of cycles of interpreting and questioning, consideration of different explanations, hypothesis and other points of view." In particular, the system proposes the features it thinks the user is using to decide whether the agent is behaving desirably. The system also proposes alternative features that the user could consider when assessing the agent's behaviour, forcing the user to consider alternative perspectives and reflect.


\subsection{Reward Modeling} \label{reward_modeling}
Once the feedback from the user(s) has been collected, the next step in the RLHF pipeline is to create a reward model that can give feedback to the learning agent on behalf of the human. The creation of a reward model that can issue rewards on behalf of humans is important as, depending on the complexity of the environment and the desired behaviour, it can take millions~\cite{pardo2018time} or even billions~\cite{agapiou2022melting} of timesteps for an agent to learn the desired behaviour. \carter{Improve transition or say more?}

\subsubsection{Trajectory Encoding}
During the feedback collection phase, the user converses with the system about how they would like the agent to act. All of the feedback collected from the user is in natural language. Thus, the reward model must be able to make use of natural language information. However, the information about the agent and environment may not be in natural language. For example, in a grid world environment, the information about the environment and the agent's actions in the environment is stored in a numerical format that can later be rendered as an RGB array when a human wants to view it. This presents a challenge as the feedback from the user and the information about what the feedback is referring to, namely the agent and the environment, are not in the same format.

One possible solution to this grounding problem is to use a vision-language model (VLM) that can accept both natural language and visual information. However, when we performed preliminary testing, we found that the performance of VLMs was notably poor when attempting to prompt the model to reason about detailed spatial information from reinforcement learning environments such as grid worlds. It is possible that as VLMs improve, they will be able to successfully reason about high-granularity spatial images. Regardless, given current capabilities, we opted to convert the trajectories into ASCII representations, which an LLM can understand.

To do so, we coded each entity in the environment with an ASCII character. For example, for the environment used in our evaluation, the main agent the user was giving feedback on was represented by an ``\texttt{M}'', apples, which the agent could collect for reward, by ``\texttt{A}'', other agents by ``\texttt{B}'', garbage by ``\texttt{G}'', empty tiles by ``\texttt{.}'', and territory boundaries by ``\texttt{-}'' and ``\texttt{|}''. We also annotated each step in the trajectory with the step number and important actions that occurred. Figure \ref{fig:ascii-encoding} shows an example of two timesteps encoded in this way. Notably, all of the information comes from the underlying state of the environment and is programmatically generated. This means a human does not have to convert and annotate each trajectory, which is important for scalability. 

\subsubsection{In-Context Language-Based Reward Model}

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/prompt_structure.png}
  \caption{\todo{Placeholder image for now. Should differentiate between diversity and uncertainty-based trajectories. } Reward model prompt structure
  }
  \Description{}
  \label{prompt_structure}
\end{figure}

The reward model can be thought of as a classifier in that it receives a trajectory, parsed into ASCII, as input and outputs $1$ if the agent's behaviour aligns with the user's expressed intent and $0$ otherwise. To achieve this, we provide an LLM with the information collected about the user during the dialogue-based preference elicitation and ask the LLM whether the agent's behaviour in the input trajectory is aligned with the user's expressed intent. If the LLM thinks the agent behaves according to the user's expressed intent, we parse this to a 1 and otherwise a 0.

To achieve this, we create a prompt that includes 
\begin{enumerate}
    \item a description of the environment and the ASCII characters used in the encoding,
    \item the information gained from the user during during the dialogue-based preference elicitation,
    \item a description informing the language model that its goal is to predict whether the agents behaviour is aligned with the user's intent,
    \item an ASCII representation of the trajectory that the model is to label,
    \item text to encourage the model to engage in chain-of-thought reasoning,
    \item and instructions about how the LLM is to format it's response so that we can parse the output.
\end{enumerate}
A high-level overview of the prompt structure is shown in figure~\ref{prompt_structure}. 

The design of this prompt was inspired by two major findings about LLM capabilities. First, LLMs have been found to be effective in-context, few-shot learners \cite{brown_language_2020}. This means that a trained LLM, with fixed parameters, can learn new patterns by including the the beginning of a pattern as context, and asking the model to continue the pattern. In settings similar to ours, this has been shown to be far more sample efficient than traditional supervised learning~\cite{kwon2022reward}. The pattern of interest in our case is what behaviour the user deems to be aligned with their intent. The second finding is that prompting LLMs to engage in chain-of-thought reasoning can greatly increase their performance~\cite{kojima2022large}. The idea is that the model forms an argument first, and then due to the auto-regressive nature of language models, uses the argument it made to determine a final answer. In other words, the LLM must justify its answer before giving it. 

Since our LLM-based reward model receives a full trajectory as input and outputs a reward, it can deal with non-Markovian rewards. This means that the reward model can evaluate the agents behaviour over multiple time steps when determining the reward. We hypothesized that this would be important for capturing user's preferred agent behaviour, and this was supported by our empirical findings presented later. For example, some user's thought that it was only respectful for an agent to enter another agents territory if that other agent had already entered their territory. This is markedly non-Markovian as it cannot be determined in a single timestep.

\subsubsection{Making the Reward Model Efficient}

While LLMs can efficiently learn language-based patterns in context, this comes at a cost. LLMs are very expensive and relatively slow to query as they have a large number of parameters. Since training an agent can require millions of training steps, solely using an LLM-based reward model could be infeasibly slow. To deal with this, our LLM-based reward model could be used to assign rewards to a pool of trajectories which could then be used to train a more efficient reward model with supervised learning. Each trajectory in the pool of trajectories labelled by the LLM-reward model would be converted to its numerical representation which would serve as the input for the supervised learning algorithm. The training labels would be the labels assigned by the LLM-based reward model.

% Our system uses reflective dialogue to elicit the user's preferences. The information gained from this is then used to do language-based reward modelling. This reward model is then used to do Reinforcement Learning from AI Feedback (RLAIF). The agent is then trained, and the user evaluates the behaviour of the trained agent and can repeat the process, thus closing the loop.

% Reflective-Dialogue-Based Preference Elicitation. Moon suggests that reflection is ``a form of mental processing with a purpose and/or an anticipated outcome that is applied to relatively complicated or unstructured ideas for which there is not an obvious solution'' (Moon, 1999, p98). In our case, we would like users to reflect on what kind of behaviour they would like an agent to embody and what that would look like. To achieve this, we explicitly program the dialogue of our system to prompt the user to reflect at various depths. Initially, the user labels whether a given trajectory acts in the right way and explains why. This  
% \subsection{Dialogue-Based Preference Elicitation}
% To begin the process, we collect a large pool of random rollouts. The agent is untrained and just taking random actions in the environment. We then need a way to narrow these down.

% Strategies from active Learning are used to decide which trajectories to show the user. We use pool-based sampling. When we have little information, we can use diversity-based sampling where we just look for some small subset of the pool that are \textit{diverse}. In our case, we perform k-means clustering on embedded vectors that represent the trajectories. We then select the centroids (center of each cluster) for the user to label. If we have more information from the user and can make a model of their preferences, then we can use uncertainty-based sampling to select the trajectories where the model is least certain. In our case, we use the token probabilities of the label from the language-based reward model to determine the trajectory which the model was least certain about. If we were trying to embed respectful behaviour into the agent, then we would look at the trajectory where, when shown to the model, the token probabilities of "respectful" and "disrespectful" are closest. Uncertainty-based sampling can help us refine a model.

% Dialogue-Based Preference Elicitation. Show dialogue flow and talk about feature-based vs item-based preferences. Could make a dialogue flow diagram. 

% Reflection
% \subsection{In-Context Language Based Reward Modelling}
% Large language models have been shown to be effective in-context learners. This is useful since it is common in inverse reinforcement learning to assume that

% We use the information gained from the user during the dialogue-based preference elicitation to create a language-based reward model.

% We parse the trajectories into an ASCII representation and save this with the user explanation. 

% We use chain of thought.
\subsection{Interactive RLHF}
Our system focuses on the feedback collection and reward modelling phases of RLHF and not the policy optimization (agent training) phase. However, once our reward model has been used to train an agent, we could restart the process. Instead of sampling trajectories where the agent is untrained we would simply sample trajectories where the agent is trained. As such, this would allow for \textit{iterative} refinement of the reward model and resulting agent. 
% For example, if the original reward model lacked information about a certain edge case, it is possible that the agent would learn undesirable behaviour in that. 



% \todo{finish up this section}
% Once the language-based reward model has been developed, we can use this to train a cheaper and faster reward function using an RNN. We take the human feedback, make a language based reward model, use this to label a moderate amount of trajectories, and then train a traditional reward model on these LLM labelled trajectories. Following this we can train an agent with the RNN reward function. We can then show the user behaviour of the \textit{trained} agent and restart the loop. The agent can be trained in a multi-objective (utilizing the alignment reward and the environment reward) or a single-objective (just using the alignment reward) fashion.

% Another benefit of making this process interactive is that we may notice that our agent is reward-hacking the "respectfulness" reward. In this case we may want to add another behavioural pattern or value to counteract this. \carter{King Midas example?}

==> versions/v1.apr.2/4_system_evaluation.tex <==
\section{Pipeline Evaluation}

To evaluate our system, \systemname{}, we measure the inter-annotator agreement between the system and the user on a test set of trajectories. We compare this to the inter-annotator agreement between the participants and to a baseline inspired by the method presented by Kwon et al.~\cite{kwon2022reward}. We also measure the system's balanced accuracy using the user's reward labels as the ground truth. We compare the balanced accuracy of our system to the baseline inspired by the method proposed by Kwon et al.~\cite{kwon2022reward}.

\subsection{Method}
We recruited 21 participants to use our system to express their understanding of respectful behaviour in a grid world environment we designed for the study. After using our system, participants labelled the behaviour of an agent in 20 trajectories as ``respectful'' or ``disrespectful.'' We converted the user's labels to binary rewards, where ``respectful'' corresponded to 1 reward and ``disrespectful'' corresponded to 0 reward. We then constructed a reward model using the information gained from the user during their dialogue with the system. Finally, we compared the binary rewards given by the reward model to the binary rewards given by the user.

\textit{\textbf{Participants}} We recruited 21 participants from our institution (18 to 39 age range, M=23.9, 7 self-identified as male and 14 as female). When asked to rate their level of familiarity with reinforcement learning on a 5-point likert ranging from ``very unfamiliar'' (1) to ``very familiar'' (5), the mean level of familiarity was 2.48, with the mode and median both being 2. The Likert data is visualized in figure \ref{fig:rl_familiar}.

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/rl_familiar.png}
  \caption{Participant familiarity with reinforcement learning}
  \Description{}
  \label{fig:rl_familiar}
\end{figure}

\textit{\textbf{Grid World Environment: }}
To ensure the reward model performed in-context learning instead of using memorized knowledge, we decided to create our own closed-source grid world environment. This ensured the LLM used in the reward model had no previous knowledge about the environment. The environment can be seen in figure \ref{fig:teaser}.

The environment is a 6$\times$6 grid world. There is one blue "main" agent in the environment and three grey ``background'' agents. The main agent is the agent the user gives feedback about. There are also, apples which the agent can pick up for reward and garbage which the agent can collect for no reward. Each one of the agents owns one of the four 3$\times$3 quadrants which each represent an orchard. Each agent is free to move around the whole grid, however two of the three background agents were programmed to be stationary. 

\textit{\textbf{Baseline:}} Kwon et al. \cite{kwon2022reward} proposed a reward modelling pipeline for text based environments where the user provides multiple examples of the agent behaving as they would desire accompanied by explanations. Our baseline is inspired by their pipeline but is slightly modified in the following way: Instead of asking the user to come up with examples, we choose the examples the user sees with the diversity-based sampling procedure described in stage 1 of section \ref{dialogue-based_preference_elicitation}.

Since the pipeline above is a subprocess of our full system, \systemname{}, the user only interacts with our system, but when forming the reward model for the baseline, we only include the information collected from the user during the first iteration of stage 1 mirroring the pipeline proposed in \cite{kwon2022reward}.

\textit{\textbf{Procedure:}} The participants used our interface to specify how they would like the agent to act via our dialogue-based preference elicitation process. Participants then labelled 20 trajectories as either ``respectful'' or ``disrespectful'' based on their own definition of respect.

\textit{Introduction ($\sim$5min)} - After completing the consent form and the demographic questions, the grid world environment mechanics were explained to the user, including explanations of each entity, the ownership of orchards, that agents could not interact or block one another, and that each agent could see the full map. Following the explanation of the environment the participant was told that they would only be evaluating the blue agent that starts in the upper left quadrant and that they should assess whether this agent acts respectfully according to their own understanding.

\textit{Dialogue} - The user began by conversing with the system about the agents behaviour following the dialogue structure presented in section \ref{dialogue-based_preference_elicitation}. For the sake of controlling the amount of time users spent on the activity, we limited the user to one preference clarification loop and one uncertainty reduction loop. 

\textit{Labelling} - Following the participants' dialogue interaction with the system, participants labelled 20 trajectories as ``respectful'' or ``disrespectful'' using 1 for respectful and 0 for disrespectful. Each participant labelled the same trajectories, which allowed us to assess how much the participants agreed on what was respectful.

\textit{Semi-structured Interview ($\sim$10min)} - After completing the labelling task, the participant was asked whether they felt they were able to give the system a good understanding of their notion of respect, if they were always able to articulate why they thought a behaviour was respectful, if it was ever difficult to decide, and if they thought their definition of respect evolved over time and what caused the change.

\subsection{Reward Modeling}\label{partic_reward_modelling}
For each participant, we constructed a baseline reward model and a reward model using our pipeline. For the baseline reward model, we used the four explained trajectories from the first iteration of the item-based preference elicitation where diversity-based sampling was used (stage 1 of section \ref{dialogue-based_preference_elicitation}). For the reward model based on our pipeline, we used all information from the dialogue-based preference elicitation. The environment description, task description, and all other aspects of the prompt remained the same for both reward models. Both reward models used GPT-3.5 Turbo.

After constructing both reward models for each participant, we used each to assign rewards to (label) each of the trajectories the user labelled during the labelling phase of the activity.

\subsection{Data Analysis}

Our analysis aims to answer two questions: First, is our reward modelling pipeline better than the baseline? Second, can \systemname{} capture individual definitions of value-aligned behaviour? 

To address the first question, we compare the balanced accuracies obtained for each user by our system to the baseline system using the Wilcoxon signed-rank test. For each participant, we convert their label (``respectful'' or ``disrespectful'') to a binary reward. The idea is that we would like the agent to act respectfully, so when the participant deems the agent has acted respectfully, the agent receives a reward of 1 and otherwise does not receive a reward. We treat the binary rewards generated by the participant as the ground truth labels. Then, for each participant, we assign binary rewards to each of the 20 trajectories they labelled with the baseline reward model and our reward model. Thus, we get a balanced accuracy score for each reward model for each participant. We chose balanced accuracy as, depending on the participant's notion of respect, the labels may have a class imbalance. We then compare the baseline reward model's balanced accuracies to our reward model's balanced accuracies using the Wilcoxon signed-rank test. We chose this test over a parametric alternative as it is less likely to produce false positives and is more robust when the distribution of the data is unknown or skewed \cite{bridge1999increasing}.

To answer the second question, we measure how much the reward models produced by each pipeline agree with the participants they are modelling. We then compare this to how much the participants agree with one another. Specifically, we created two reward models for each participant: one using the baseline pipeline and another using our pipeline (as described in section \ref{partic_reward_modelling}). We assess the agreement between each participant's responses and their corresponding reward models using the Fleiss' kappa metric. By averaging these agreement scores across all participants for both pipelines, we obtain a measure of how well the reward models from each pipeline match the participants' views. We also bootstrap the agreement scores to obtain confidence intervals for the average agreement between the participants and the reward models from each pipeline. We then calculate the inter-annotator agreement between all participants again using Fleiss' kappa. \todo{add citation and explanation for the choice of Fleiss' kappa. Maybe add a word of warning?}

\subsection{Results}

On average participants took 15 minutes 58 seconds ($\sigma =$ 6 min. 33 sec., range: 7 min. 5 sec. - 31 min. 2 sec.) to complete the dialogue with the system and 6 minutes 33 seconds ($\sigma =$ 1 min. 24 sec., range: 2 min. 23 sec. - 8 min. 31 sec.) to complete the labelling. Of 21 participants, 7 chose to enter the \textit{preference clarification loop} for one iteration.

\subsubsection{Comparison to Baseline: Balanced Accuracy}
On average, the reward models produced by our pipeline received significantly higher balanced accuracy scores (measured in percentages) than the baseline system by 7.00\% (95\% CI: [1.97\%, 12.39\%], $\mu = 71.32\%$ vs. $\mu = 64.33\%$, p=0.0240). \carter{Add table and/or bar plot?}

\subsubsection{Capturing Individual Definitions of Respect: Fleiss' Kappa}
We observed a Fleiss' kappa value between all participants' labels on the 20 test trajectories of $\kappa = 0.23$, indicating ``fair'' agreement among participants \cite{landis1977measurement}. Generally, kappa statistics below 0 indicate ``poor'' agreement and kappa statistics above 0.8 indicate ``nearly perfect'' agreement \cite{landis1977measurement}. The Fleiss' kappa statistic of 0.23 we observed lends credence to the idea that human values and preferences are subjective and personal.

The average Fleiss' kappa statistic for the reward models generated with the baseline system and the participants was $\kappa = 0.25$ (95\% CI:[0.14, 0.35]), indicating. The average Fleiss' kappa for the reward models generated with our pipeline and the participants was $\kappa = 0.36$ (95\% CI:[0.28, 0.43]).

This result indicates that the reward models produced by our pipeline, using \systemname{}, on average, agree more with each participant than the participants agree with each other about what agent behaviour is respectful. \carter{However, this result should be taken with caution?}

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/gpt35_inter-annotator.png}
  \caption{Average inter-annotator agreement between the system and participants measure by Fleiss' $\kappa$ (Exp., Exp. + Ref., Exp. + Ref. + Unc. Red.). Inter-annotator agreement between all participants (Participant Pool).}
  \Description{}
\end{figure}


==> versions/v1.apr.2/5_qualitative_analysis.tex <==
\section{Qualitative Analysis}

\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{figures/respect_features.png}
  \caption{\todo{placeholder } Behavioural features participants used to decide whether the agent was acting respectfully}
  \Description{}
  \label{respect_features}
\end{figure*}

\textbf{Evolving Understanding of Respect}.
A recurrent theme across several participants (e.g., P19, P10, P7) was an initial simplistic definition of respect, often tied to spatial boundaries or specific actions like collecting one's own apples or staying within one's quadrant.

For many participants (e.g., P19, P18, P10), their definition of respect evolved through interaction with the system. This evolution was prompted by seeing examples, receiving system feedback, and reflecting on alternative definitions presented by the system.

\textbf{Complexity in Defining Respectful Behavior}.
Several participants (e.g., P12, P17, P15) faced difficulty in labelling actions as strictly respectful or disrespectful, indicating the complex nature of respect that cannot always be boiled down to binary decisions.
Participants like P1 and P17 applied specific criteria or logic to decide on what constitutes respect. 

\textbf{Role of System Feedback and Hypotheses}.
The system's hypothesis and the presentation of alternative features influenced participants' understanding and definition of respect (e.g., P18, P13, P3). It helped some participants narrow down their definitions or consider aspects they hadn't initially thought of. While the system's alternative definitions helped refine participants' understanding, they were not always successful in changing participants' minds about what constitutes respectful behaviour (e.g., P19).

\textbf{Impact of Examples and Interaction}.
Interaction with the system and exposure to examples played an important role in clarifying and refining participants' definitions of respect (e.g., P18, P20). It helped participants articulate their thoughts more clearly and consider behaviours they hadn't initially.
Participants P1 and P11 found it hard to label actions that seemed neutral, highlighting the existence of grey areas in defining respectful or disrespectful behaviour.

\textbf{Personalized Definitions and Intuition}.
The data shows a wide variability in how participants defined respect, with some relying on intuitive understandings that evolved over time (e.g., P6, P4). Participants consistently noted the difficulty in classifying actions that did not clearly align with their definitions of respect, indicating a need for a "neutral" category or more nuanced labelling options.



\subsection{Definitions of Respect}\label{definitions_of_respect}
We analyzed the conversations the user had with the system to understand what each participant thought respectful behaviour in this environment was. We found 12 behavioural features that participants used to explain whether they thought the agent was respectful. Interestingly, P1 only used one behavioural feature, namely whether the agent stayed in the quadrant it owned, to determine whether the agent acted respectfully. In contrast, P5, P7, and P10 explained whether the agent was acting respectfully using seven features over the course of the dialogue. Overall, no two participants used the same set of features to make their decisions. Further, participants combined the features in diverse ways, such as forming hierarchies of importance or combining them conditionally.

The 12 features we identified are:
\begin{enumerate}
    \item \textbf{Stays in Own Quadrant:} Whether the main agent stays in the orchard (quadrant) they own.
    \item \textbf{Interferes With Others:} This feature evaluates a relatively wide range of behaviours including if the agent appeared to attempt to block another agent, following another agent, getting to close to another agent.
    \item \textbf{Task Completion:} Whether the agent works toward or completes the task the participant thought the agent should be doing. For example, an agent picking up all apples or garbage in their quadrant. 
    \item \textbf{Picks Up Own Garbage:} Whether the agent picks up garbage in their own orchard (quadrant)
    \item \textbf{Picks Up Others' Garbage:} Whether the agent picks up garbage in other agents orchards
    \item \textbf{Tit for Tat Behaviour: }Some participants explained that a given behaviour was respectful if another agent had done it to them first, such as entering their quadrant.
    \item \textbf{Taking Others' Apples}: Whether the agent picks up apples in orchards it does not own.
    \item \textbf{Eats Own Apples: }Whether the agent eats any apples in their own quadrant.
    \item \textbf{Picks Up Garbage Before Apple:} Whether the agent picks up garbage before eating apples in their own or other quadrants.
    \item \textbf{Efficiency: }Whether the agent moves around without collecting apples or garbage or makes repetitive, futile movements
    \item \textbf{Time in Others' Quadrants:} The duration of time spent in other agents' orchards.
    \item \textbf{In Quadrant While Owner was Gone: }If the agent entered another agents quadrant while they were gone.
\end{enumerate}

Among the features, the most commonly used was \textbf{Stays in Own Quadrant}, but participants often found other features more important. Some features are temporally static while others span multiple steps. For example whether an agent is in its quadrant can be determined at a single time, but whether an agent picked up garbage before eating an apple must be determined over multiple steps. The features each participant used are shown in figure \ref{respect_features}.














 

% \begin{itemize}
%     \item Multiple participants seemed to want to factor in efficiency or task performance into their definition of respect. I think there may be some implicit understanding that the "right" thing to do in games is get a high score. However, one user said they noticed this about themselves and consciously focused on not letting this determine their respectful labels. Another participant said that since the agent gets reward for picking up apples, this must be a task that the designer wanted the agent to do. Thus reward maximizing while staying in the quadrant is the nice thing to do.
%     \item Multiple users noted that seeing the system's understanding of their definition of respect and also the other factors that could be considered helped them understand their definition. This could be related to the participants asking the researcher what the definition of respect was. It seems as though some participants are not sure about their own definition of a value and need help reflecting. 
%     \item One participant pointed out the agents that did not move. They mentioned that it was difficult to evaluate if the main blue agent was acting disrespectfully when it took their apples because it seemed like they didn't want the apples anyway. 
%     \item One participant noted that if the main agent went into the quadrant owned by an agent that had entered the main agent's quadrant, this was respectful. They mentioned that it was a kind of tit-for-tat. 
%     \item A main theme seems to be that of efficiency vs. respect. Some think they are opposed and some think that they almost mean the same thing, and yet others think that they are not related at all (some said respect was just based on boundaries).
    
% \end{itemize}

==> versions/v1.apr.2/6_discussion.tex <==
\section{Discussion and Future Work}

Here we discuss and reflect on important findings from the development and evaluations of \systemname{}, we note limitations, and oppertunities for future work. 

\subsubsection*{The Diversity of Values} We developed our system based on the hypothesis that human values and individual's undertandings of humans values are diverse. We were motivated by cases where people would want an agent to embody \textit{their} specific definition of a value; for example, an agent operating in someone's home.

When asked to train an agent to act respectfully according their own understanding, participants used vastly different behavioural features to explain whether or not the agent was acting respectfully. We identified 12 different behavioural features that participants based their explanations on. Each participant used a different subset of behavioural features and combined them in unique ways. This clearly reflects the idea that different people have different understandings of human values. If you were to train an agent with one of the participants definitions of respect, the agent would likely not align with another participants definition. For example, if a company decided that making household humanoid robots respectful was important, and trained it to be generally respectful, the end users may not find the behaviour only minimally respectful. As such, we reiterate that an accesible interface that allows end users and people without reinforcement learning experience to align agents to their individuals is imperative.

Our qualitative results on the diversity of participants definitions of respect is supported by our analysis of the inter-annotator agreement between the participants when labelling videos as respectful or not. In particular, we only found ``fair'' agreement between participants ($\kappa = 0.23$).

\subsubsection*{Non-Markovian Behavioural Features}
We found that some of the features used by participants to determine whether the agents behaviour is respectful violate the Markov property. This means that the behavioural feature could not be assesed in the current time step alone. An example of a feature that \textit{does} satisfy the Markov property is whether the agent is in it's own orchard - the current state holds all the information necessary to determine the feature. An example of a behavioural feature that violates the Markov property is whether or not the agent picked up garbage \textit{before} collecting an apple. This feature requires information from at least two states to be determined. Similarly, some participants considered whether an agent went into the quadrant of another agent that had already been in their quadrant (feature 6 in section \ref{definitions_of_respect}).

Since some of the features participants used are non-Markovian, it is important to have a reward model that can capture this. If, for example, the reward model only receives a single step as input (as is common in traditional RL), these non-Markovian features cannot be captured. The reward models produced by our pipeline take as input an entire trajectory. While this can be less precise, it allows for the use of non-Markovian features to be used in determining the reward. 

\subsubsection*{The Importance of Reflection}
When comparing our system/pipeline to the baseline that does not rely on reflection, we found that our system significantly outperformed the baseline. This points to the fact that encouraging the user to consider alternative perspectives and reflect on their preferences allows them to more clearly communicate their intent to the system. 

The qualitative results also support this conclusion. Many participants (P3, P4, P9, P13, P16, P18, P20, P21) noted that seeing and responding to the hypothesis proposed by the system about what features they were using to determine if the agent was acting respectfully and the alternative features, allowed them to either refine, better explain, or clarify their own understanding of respectful behaviour in this environment.

\subsubsection*{Generation vs. Evaluation}
Previous work on using natural language reward models by Kwon et al.~\cite{kwon2022reward} prompted users to come up with come up with examples of the behaviour they would like the agent to embody. While this gives the user a high degree of control, we overwhelmingly found that participants did not initially know what behaviours they thought were respectful. Participants mentioned that just seeing various trajectories of the agent behaving in the environment allowed them to better understand what they thought was respectful. Further they found that the system's hypothesis and proposition of alternative features was useful for framing and clarifying their thinking.

In sum, our results point to the fact that giving the user examples to evaluate will likely lead to more accurate reward models compared to having the user generate examples on their own.


\subsubsection{Accessibility}
In some cases, people may want to train agents to align with their individual values and preferences. For example, users may want AI systems in their home to align with their or their families values. As such, there is a need for accessible solutions for aligning agents to individual values. In our study, a majority of the participants were either ``very unfamiliar'' or ``unfamiliar'' with reinforcement learning and yet the system was still able to capture their definition of respect, allowing them to create a reward model that could be used to train an agent. 

 \subsection{Ethical Considerations}
 While personalization of AI systems and agents has clear advantages, there are also risks. Due to the inherent diversity of values and preferences, in some cases aligning to one person's preferences means unaligning from others'. For example, if one person believes that it is respectful for their agent to pick up garbage on their neighbours property, but the neighbour does not believe this is respectful, a case inspired by the results of our evaluation. Problems such as this are faced by human societies and we have developed solutions, but solutions suitable for governing humans may not be suitable for govering AI agents. \todo{Finish thought with something about AI regulation} 

Further, while we exemplified the use of our system, \systemname{}, for aligning agents to respectful behaviour, we acknowledge that the system could be used to train agents with more nefarious values. Because of this, before deploying a system for personalizing AI agents, it is important to build guard rails that limit the range of possible behaviours that can be trained into the agent.

\subsection{Limitations}

\subsubsection{Implementation Dependence}

Some aspects of our system are artifacts resulting from the current capabilities of large language models and large vision language models. For example, we textually encode trajectories so that they can be input to a language model. We made this choice as vision language models performed poorly on the grid world environment we developed. However, in the future, this may not be necessary as capabilities of LLMs and VLMs increase. With that being said, while some aspects of the system are model dependent, the core of the system, namely the overall pipeline, is not model dependent and as capabilities increase, we expect the performance of the pipeline to only increase. 

\subsubsection*{Reward Model vs. Agent Accuracy}
We focused our system and evaluation on the feedback collection and reward modelling phases of the RLHF pipeline and did not consider policy optimization (agent training). We made this choice because our core innovation is not related to policy optimization. This leaves questions open about the behaviour that would result from training an agent with a reward model produced by our system. However, Kwon et al. \cite{kwon2022reward} found that RL agent accuracy mimics the reward model accuracy.

\subsubsection*{Binary Labels}
 Multiple participants mentioned that it was difficult to classify some trajectories as either respectful or disrespectful and that some seemed neutral. As such, the fact that our system uses binary reward could be seen as a drawback. 
 % In RLHF it is common to use pairwise comparisons where participants would, for example, decide which of two options is ``more respectful.''
 
\subsubsection*{Environment Complexity}
The environment we used to evaluate our system is relatively simple and abstract. While we believe we are the first to implement language rewards in a grid world, the more realistic environments may present new challenges. 

\subsection{Future Work}
While our system takes a step in the right direction, we are still far from solving individual alignment. There are likely many possible interface improvements that would make the system more usable and accessible, and algorithmic improvements which would make our system more performant. With that being said, our system can be seen as a baseline for other HCI researchers that can be used as a point of reference.

\subsubsection*{Integration of Pairwise Comparisons}
Pairwise comparisons can be useful for eliciting preferences as they allow annotators to make relative assessments as opposed to absolute assessments. Integrating pairwise comparisons into the dialogue-based preference elicitation phase of our system could help address the difficulty some participants had in deciding between binary labels.

\subsubsection*{More Values in More Realistic Environments}
We evaluated our the efficacy of our system in capturing individual user's definitions of respect in a multi-agent grid world environment. Future work could adapt the system to more realistic environments. It could be the case that VLMs work be more effective in more complex environments as the data is likely closer to the distribution of the training data.
 


==> versions/v1.apr.2/7_conclusion.tex <==
\section{Conclusion}

We developed a system, \systemname{}, that allows users with no particular experience in machine learning to train agent's in alignment with their individual values and preferences. In a user study where participants evaluated whether an agent's behaviour was respectful or not, we found that different people have vastly different definitions of what respectful behaviour is. Further, we found that our system was able to capture each individual's definition of such behaviour to a relatively high degree of accuracy.

==> versions/v2.sep.10/1_introduction.tex <==
\section{Introduction}
%\carter{Emphasize the relationship between alignment and reward modelling?}
As AI systems and agents take on more tasks and affect personal parts of our lives, it is increasingly important to align their behaviour with human values at both individual and collective levels. This alignment challenge spans from personalized interactions, like an AI agent's respectful behaviour in a household, to broader societal collective decisions.

Current AI alignment approaches, such as reinforcement learning from human feedback (RLHF), often rely on feedback aggregated from many users \cite{casper_open_nodate, bai_training_2022}. This aggregation implicitly makes collective decisions about AI behaviour, potentially marginalizing minority viewpoints or unique preferences \cite{siththaranjan2023distributional}. By "averaging out" personal differences, these methods risk creating systems that ignore the values of minority groups or those with uncommon preferences. Accurate individual reward models offer a solution to this problem. These models enable personalization by tailoring AI behaviour to each user's unique values and beliefs when appropriate while simultaneously providing a foundation for more representative and interpretable collective decision-making. By understanding individual stakeholder preferences, we can aggregate diverse viewpoints more fairly and make informed trade-offs in group contexts. This approach addresses both the need for personalized AI interactions and the challenge of making ethical collective decisions.

However, creating personalized reward models presents several challenges. First, finding the most effective way for humans to convey their goals and desires to AI systems remains an open question \cite{casper_open_nodate}. Second, end users of AI systems may lack the technical skills or necessary training to provide feedback to an agent \cite{bai_constitutional_2022}. Third, it is impractical to expect individuals to teach an agent how to behave when many examples may be required.

In this work, we present \systemname{}, an interactive system for aligning AI agents to individual values that is novice-friendly and sample-efficient. The user-facing side is a simple chat interface that prompts users to explain their desired behavioural patterns and selectively sends examples of the agent's behaviour to solicit feedback using active learning techniques \cite{mosqueira-rey_human---loop_2023}. The system's textual messages are designed to encourage users to reflect deeply on their value definitions, inspired by prior work on designing for reflection \cite{fleck2010reflecting, wolfbauer_script_2022, kocielnik_reflection_2018, bentvelzen_revisiting_2022}. Using the feedback gathered from the dialogue, we create a language-based reward model that leverages the in-context learning abilities of large language models \cite{brown_language_2020}.

We evaluated \systemname{} through two studies involving a total of 30 participants. In the first study, 21 participants used the system to build a reward model for their personal definitions of respectful behaviour. The second study involved 9 participants and focused on ethical decision-making in autonomous vehicles. We found that participants had widely varying definitions of value-aligned behaviour across both studies and that our system could capture these subjective and personal definitions significantly more accurately than baseline systems.

Our contributions are as follows:
\begin{itemize}[topsep=0pt]
\item A novel, accessible, and theoretically grounded pipeline for aligning AI agents to individual values and preferences, drawing upon insights from AI, HCI, and social science research.
\item A comprehensive evaluation of the system across two distinct domains, demonstrating its ability to capture individual human values and ethical preferences.
\item Empirical evidence highlighting the diversity of individual interpretations of value-aligned behaviour.
\item Insights for future work on enabling end users to interactively align AI agents with their personal values, including potential applications in both individual and collective alignment contexts.
\end{itemize}
% As AI systems and agents take on more tasks and affect personal parts of our lives, it is increasingly important for us to be aware of the values that they possess and who decides what these values should be. Take, for example, the desire for respectful interaction from an AI agent within a household. The agent's behaviour should align with the unique interpretation of {\it respect} held by the individual or family using it, as another person's conception of respect might vary widely based on their background and beliefs. 
% % Moreover, in scenarios where AI systems need to make decisions affecting multiple individuals or groups, there's a need for methods that can aggregate diverse individual preferences into collective decisions.

% Reinforcement learning from human feedback (RLHF) has recently emerged as a popular and effective method for aligning AI systems to human goals and desires~\cite{casper_open_nodate}, but the feedback generally used in this process is aggregated from many individuals \cite{bai_training_2022}. In aggregating feedback, personal differences in beliefs about how an agent should act are ``averaged'' out, which can lead to systems that ignore the values of minority groups or those with uncommon or unique preferences~\cite{siththaranjan2023distributional}. Hence, in constructing value-aligned behaviour, AI systems and agents are usually either aligned to an aggregated group definition of desirable behaviour (through large-scale human-feedback data collection) or to the system designer's definition, as in traditional reinforcement learning systems. 

% % \subsection{What are we trying to do and why is it relevant?}
% %How should AI agents act? There is no single universally satisfying answer to this question, as people have diverse preferences and values that are shaped by their personal backgrounds. 

% %This requires an accessible way for users of AI systems to express their desires and goals to the system and an effective way to model these desires and goals so that they can be incorporated and embedded into AI systems and agents.


% % It has been acknowledged in the AI community that the best method for humans to interact with the system to express their goals and desires is still an open problem in human-computer interaction\cite{casper_open_nodate}. The solution for doing this needs to be accessible, as people without expertise in machine learning may wish to use AI systems to their desires. For example, imagine a person who purchases a humanoid robot to do household chores and wants the robot to act respectfully in their home according to their definition of respect. As part of being accessible, the system must be sample-efficient and minimally time-consuming, as people may not have days of free time to teach an AI system how to act appropriately. And the system must accurately capture the given individuals' desires and preferences.

% % \subsection{Why is it hard?}
% % \carter{Clear up this paragraph.}
% Since the way individuals define values is subjective and personal, there is a need for a personalized and efficient way for end users to tailor AI behavior to reflect their unique interpretation of values. To make this possible, there are several challenges that must be addressed.
% % desired behaviours associated with a human value and train agents to act accordingly.
% % However, this problem is challenging in a number of ways.  For example, while reinforcement learning from human feedback (RLHF) is a promising method, it has been acknowledged in the AI community that the best method for humans to communicate goals and desires to the system remains an open problem~\cite{casper_open_nodate}. Novice users also may not have the technical know-how or the necessary training on how to give feedback to an agent~\cite{bai_training_2022}. Finally, it is completely impractical to demand individuals to teach an agent how to behave, when tens of thousands of examples may be required.
% First, although reinforcement learning from human feedback (RLHF) is a promising approach, it has been recognized that finding the most effective way for humans to convey their goals and desires to AI systems is still an open question~\cite{casper_open_nodate}. Second, end users of AI systems may not have technical skills or the necessary training on how to give feedback to an agent~\cite{bai_constitutional_2022}. Third, it is impractical to demand individuals to teach an agent how to behave when an extensive amount of examples may be required. 

% % \subsection{How do we solve it?}
% In this work, we present \systemname{}, an interactive system for learning about an individual's preferences that is personalized, novice-friendly and highly sample-efficient. The user-facing side is a simple chat interface through which the system prompts the user to explain the behavioural pattern they would like the agent to embody and selectively sends examples of the agent's behaviour to the user to solicit their feedback using active learning techniques~\cite{mosqueira-rey_human---loop_2023}. %We choose the videos to collect feedback on using techniques from active learning, an area of human-in-the-loop machine learning \cite{mosqueira-rey_human---loop_2023}. 
% % In particular, we use diversity- and uncertain-based sampling methods to select videos that demonstrate diverse agent behaviour in order to solicit feedback on cases that are most likely to challenge the user's concept of value-aligned behaviour. 
% The system's textual messages are designed to encourage the user to reflect and think deeply about their value definitions and preferences and are inspired by prior work on designing for reflection \cite{fleck2010reflecting, wolfbauer_script_2022, kocielnik_reflection_2018, bentvelzen_revisiting_2022}. Using the feedback gathered from the dialogue, we create a language-based reward model that relies on the in-context learning abilities of large language models~\cite{brown_language_2020}. 
% % \subsection{How do we verify we solved it?}

% We evaluated \systemname{} through two studies involving a total of 30 participants. In the first study, 21 participants used the system to build a reward model for their personal definitions of respectful behaviour. The second study involved 9 participants and focused on ethical decision-making in autonomous vehicles. We found that participants had widely varying definitions of value-aligned behaviour across both studies and that our system could capture these subjective and personal definitions significantly more accurately than baseline systems.

% Our contributions are as follows:
% % \begin{itemize}[leftmargin=*]
% \begin{itemize}
% \item A novel, accessible, and theoretically grounded pipeline for aligning AI agents to individual values and preferences, drawing upon insights from AI, HCI, and social science research.
% \item A comprehensive evaluation of the system across two distinct domains, demonstrating its ability to capture individual human values and ethical preferences.
% \item Empirical evidence highlighting the diversity of individual interpretations of value-aligned behaviour and the effectiveness of our approach in capturing these nuanced perspectives.
% \item Insights for future work on enabling end users to interactively align AI agents with their personal values, including potential applications in both individual and collective alignment contexts.
% \end{itemize}

% We evaluated \systemname{} with a 21-user study where participants used the system to build a reward model for their own personal definitions of respectful behaviour. We found that participants had widely varying definitions of respectful behaviour and that our system could capture these subjective and personal definitions of such behaviour significantly more accurately than a baseline system.
% inspired by Kwon et al.~\cite{kwon2022reward}.
% We found that the reward model generated by our system aligns more closely with an individual user's actual reward model than the alignment observed among different participants. This suggests that our system can more accurately predict a user's perception of an agent's respectful behaviour compared to predictions made by another individual using their own understanding of respect. 
% We also compare our system to a baseline inspired by \cite{kwon2022reward}, where only explained examples are used to generate a reward model on the user's behalf. Results show that our system significantly outperforms the baseline in capturing individual human preferences. 

% \subsection{Contributions}
% Our contributions are as follows:
% \begin{itemize}[leftmargin=*] 
%     \item A novel, accessible and theoretically grounded pipeline for aligning AI agents to individual values and preferences that draws upon insights from  AI, HCI, and social science research.
%     \item An evaluation of the system that demonstrates its ability to capture individual human values.
%     % \item The introduction of an important and under-studied question in HCI: How to best collect human feedback for RLHF
%     \item Insights for future work on how to enable end users to align AI agents with their personal values interactively.

    % how to enable end users to interact with agents in a way that aligns these agents with their values.
    % \item We 
    % \item We successfully implement language-based rewards in grid world environments
% \end{itemize}

% In the remainder of our paper, we introduce

%Our system does not solve the problem of individual value alignment but takes a step towards a solution. We hope this work inspires other HCI researchers to work on this difficult problem.

% \carter{Old below}
% Hook argument: Values are personal and subjective. Different people will have different ideas about what is respectful or appropriate. As such, if we train monolithic systems that try to satisfy everyone, we will end up disappointing some people. The current approach to aligning large AI systems to human values aggregates over many people and aligns to the majority. If robots or AI systems are in the home, then people will want the agent aligned to their own definition of what is respectful, not an average definition or the definition of some system designer. People need an accessible lever to shape the behaviour of agents to their liking and personalize them to align with their own definitions of values. Reinforcement learning is a common approach to training agents. We can use rewards to shape the behaviour of agents, but a person cannot sit around all day, labelling examples of acceptable behaviour. Our system must be accessible, sample efficient (low effort), scaleable, and accurate capture the users personal subjective definition of a desireable behaviour pattern or value. 

% Human preferences and values are diverse among different people. 

% \carter{Old below}

% Human social values can help guide \textit{human} decision-making to favourable outcomes \cite{ravlin1987effect}. However, we are offloading ever more of our decisions to artificial intelligence (AI). As such, we may want AI agents to embody the same desirable social values as humans do. Ravlin and Meglino define social values as "general modes of behaviour that an individual 'should' or 'ought' to exhibit. In short, we can think of social values as complex behaviours or behavioural patterns that are favourable to society. For example, we may want the AI agents we train to be respectful or embody environmental behaviour.

% However, historically, it has been found to be difficult to get AI agents to reliably embody even well-defined and relatively simple behavioural patterns (amodei and olah, 2016). In reinforcement learning, the main approach used to train AI agents that will continuously interact and learn from an environment, the designer of the agent must come up with a reward function that defines desirable behaviour and rewards the learning agent accordingly. If the designer fails to align the reward signal to the desired behaviour, "reward hacking" can occur where the agent learns some behaviour that receives a high reward but which betrays the designer's intent. As a simple example, imagine that the designer of a floor-cleaning robot gives the robot a reward for sweeping up dirt. On the surface, this does not seem like a bad reward signal since sweeping up dirt should make the floor cleaner. However, the agent may learn to throw copious amounts of dirt on the floor in order to clean it up and receive a reward. Underspecified reward function is the cause. 

% While designing rewards for simple and well-defined behaviours like cleaning the floor can be difficult, the problem of reward design only becomes more difficult as the desired behaviour becomes more abstract. Human values are abstract, and different people may have different definitions of certain values. This makes designing reward functions that reliably incentivize value-aligned behaviour even more difficult. 

% Traditional function-based reward functions may have a difficult time capturing values, as values can be defined as a behavioural pattern, not an atomic action or state. This violates the Markov property, so value driven reward may need to be non-Markovian (Wirth Survey, 2017). Further, traditional function-based reward function design is extremely inaccessible, and the task is usually only undertaken by a single individual or a small group of individuals. This is because traditional reward design is difficult to do an is often thought of as more of an art than a science. This is generally undesirable as it means a small number of people get to choose how an agent that could interact with many people will behave. Lastly, traditional reward functions are notably inflexible, which can make them more susceptible to reward-hacking.

% More modern model-based approaches to reward design use machine learning to learn a reward model. This allows for a more nuanced and flexible reward function as the function is learned as opposed to hard-coded. Two common approaches are inverse reinforcement learning (IRL) and reinforcement learning from human feedback (RLHF). In IRL, the reward model is learned from expert (usually) human demonstrations. The goal is to infer what reward function the agent in the demonstrations is following, assuming the actions taken in the demonstration are optimal with respect to the hidden reward function. This approach can be effective but usually requires thousands of demonstrations. Further, IRL usually learns from a pool of trajectories and cannot obtain new feedback in the face of uncertainty (Wirth Survey, 2017).  In RLHF, human feedback on the actions of an agent is elicited, then the feedback and action data are used to learn a model of which actions a human finds desirable. Generally, both approaches require many, many samples to learn the reward model, which can be expensive or, in some cases, infeasible. Even for simple tasks, RLHF can require 700 user-labeled examples (Christiano et al., 2017), and for more complex tasks, this approach can require hundreds of thousands of human-annotated examples (Bai et al., 2022). Both of these approaches assume the humans being learned from have a perfect understanding of their own preferences which is not always the case (NEED GOOD FOUNDATIONAL CITATION FROM PREFERENCE ELICITATION LIT)

% RLHF in particular is the most popular approach to align agents with human values. A recent survey on the topic noted that many of the open questions in regard to RLHF have to do with human-computer interaction.  In particular they note, "Specifically, it is unclear what type of feedback (or combination thereof) is optimal for learning human goals, precisely how biases harm the quality of feedback, and how to best select and train human evaluators. As discussed in Section 3, human desires are difficult to express with a reward function (Skalse and Abate, 2022b; Bowling et al., 2023; Vamplew et al., 2022)" They also note that "An individual human’s values are difficult to represent with a reward function." They also note that "Using language, humans can convey a large amount of information per evaluation, reducing ambiguity and goal misspecification." They also note that ". However, AI-generated feedback has drawbacks. Humans often disagree with AI feedback. The rate of human/AI disagreement will vary by task, but Perez et al. (2022b), Casper et al. (2023b), and Lee et al. (2023) found this to happen up to 10\%, 46\%, and 22\% of the time respectively in different experiments."

% RLHF creates a massive joint reward model which requires many many data points and averages over individuals in undesirable ways. Traditional RLHF cannot be personalized because it requires so many data points. this means that some users can get averaged over in undesireable ways (DPL). \carter{Should differentiate between RLHF in general and RLHF for language models}

% If we want to make it personalized, it must be accessible. 

% In order to make reward design more accessible and more able to capture individual human values, we developed a language-based pipeline for reward design that doesn't require the designer to possess any special knowledge. Our approach allows for \textit{anyone} to train an agent to embody a value like respect.

% We leverage reflective techniques from HCI to allow users to better understand their own preferences and values. (to increase accuracy and decrease bias). In particular, we base the reflection on the levels of reflection proposed in \cite{fleck2010reflecting}. Level 1 reflection is defined as a reflective description where the
% Reflection has been found to reduce bias (cite bias), and increase accuracy (cite medical papers). 

% We leverage dialogue-based preference elicitation to capture information about the user's preferences that can be used for a language-based reward model. We couple reflection with both item-based and feature-based preference elicitation to better understand users' preferences (Priyogi, 2019).

% We use active learning with both diversity-based and uncertainty-based sampling to select good items (trajectories) for the user to label (Mosqueira-Rey et al., 2023)

% We leverage the textual preference information from the dialogue-based preference elicitation and LLM's in-context learning ability (Language Models are Few-Shot Learners, 2020) to develop a language-based reward model.

% We employ multiple feedback loops to allow for iterative reflection and refinement

% Lastly, we have an interactive approach which leverages interleaved preference query generation (Wirth Survey, 2017)

% Most other language-based reward systems are computationally inefficient due to the size of LLMs and the expense of querying them. In order to overcome with we leverage the reward model built with RLHF to train an SL (RNN) reward function using RLAIF.  Talk about improved efficiency and scalable oversight. (hierarchy of scalable oversight: human < llm < rnn)

% Value sensitive design

% from "Fundamental issues with RLHF paper":
% \begin{itemize}
%     \item three main parts of RLHF: "preference elicitation, fitting a reward model, and policy optimization" (p 18)
%     \begin{itemize}
%         \item We focus only on preference elicitation and fitting a reward model.
%     \end{itemize}
% \end{itemize}

% Talk about how LLM reward function are expensive and thus are not scalable. (SCALABLE SUPERVISION IS IMPORTANT - concrete problems in AI safety. Amodei and Olah et al.)

% Contributions:
% \begin{itemize}
%     \item a pipeline for integrating values into an AI agent
%     \item (weak)?? Environment for value learning?
%     \item (weak)?? Evaluation of inter-labeler disagreement on values
%     \item (weak)?? Connecting VSD, Reflection, DBPE, AL, IML, ICLBRM, (I)-RLHF opening the door to new fruitful collaborations and interdisciplinary research.
%     \item We are the first to use a combination of script-based dialogue and LLM text for reflection.
% \end{itemize}
% \section{Related Work}
% Value alignment

==> versions/v2.sep.10/2_background.tex <==
\section{Background and Related Work}

Our work intersects human-computer interaction, reinforcement learning, and value alignment. We draw on insights from AI, HCI, and social science research to develop a system that accurately captures individual values in a reward model. Below, we outline the related work most relevant to our system and provide the necessary background to understand it.

\subsection{Human Values and Fuzzy Decisions}
Values are principles that guide human behaviour and ethical judgments \cite{schwartz1992universals}. Friedman et al. describe values as ``what a person or group of people consider important in life'' \cite{friedman2013value}. In the context of AI systems, values can manifest in various ways. For example, in a household setting, the value of respect might manifest as an AI assistant using appropriate language or maintaining privacy. In the context of autonomous vehicles, values might include prioritizing passenger safety while also considering the welfare of pedestrians and other road users. Importantly, values vary across cultures, individuals, and contexts \cite{le2009values}. 

While values themselves may be clearly stated, their interpretation and application often become fuzzy when considered in specific contexts \cite{van2013translating}. Translating these human values into computational terms for AI systems is challenging \cite{russell2019human}. Users may struggle to articulate their values or determine which AI behaviours align with their intent.

The concept of fuzzy preferences \cite{bellman1970decision, ribeiro1996fuzzy} provides insight into this challenge. Fuzzy decision-making acknowledges that preferences, attributes, and objectives in decision processes can be imprecise. In AI alignment, this fuzziness manifests in the difficulty of precisely defining and measuring value alignment. Users may not have clear, a priori knowledge of what constitutes aligned behaviour, and the importance of different behavioural features may be unclear or change based on context.

Our work addresses these challenges by developing a system that helps users articulate and refine their fuzzy value definitions, enabling more precise alignment of AI systems with individual human values.

\subsection{Designing for Reflection}
Reflection has several notable benefits that can help users clarify their understanding of their preferences and values. For example, it has been found that prompting medical practitioners to reflect can increase diagnostic accuracy \cite{costa2019effects, fernandes2021adding, mamede2008effects}. Moreover, in consumer research, it has been found that prompting consumers to engage in preference self-reflection can lead to more accurate reporting of preferences and that engaging consumers in realistic decisions can increase preference elicitation accuracy \cite{hauser2014self}.

Designing for reflection has been of interest to HCI researchers for some time \cite{price2003new, yukawa2003co, rogers2006framework, lindstrom2006affective, ghajargar2018designing}. Fleck \& Fitzpatrick propose a framework for designing for reflection that includes definitions of various levels of reflection and techniques for supporting reflection \cite{fleck2010reflecting}. They define five levels of reflection, ranging from simply revisiting past events to critical reflection that considers wider social or moral contexts.

The recent rise of LLMs and their chat interfaces presents the opportunity for more tailored and dynamic dialogue to engage users in reflection. Some work has explored the use of LLMs for generating reflective prompts in a design template \cite{yin_jamplate_2024}, while others have used language prompts to engage users in reflection through single questions or sentence starters \cite{fessl2017known, renner2016effects, williams2016revising, ifenthaler2012determining}. Further extensions of this approach have included the use of pre-scripted, multi-message dialogues to facilitate a guided reflective process \cite{kocielnik2018reflection, wolfbauer2022script}.

We extend this body of work by integrating reflective dialogue techniques with large language models, creating a dynamic and personalized reflection process that helps users clarify their values for AI alignment.


\subsection{Reinforcement Learning and Its Variants}
Reinforcement Learning (RL) is a branch of machine learning in which an agent learns a policy, i.e., a strategy for selecting actions in an environment, to maximize the rewards it receives. Traditionally, the agent designer crafts a reward function to incentivize desirable behaviour. However, reward design is notoriously challenging and can result in reward hacking where an agent learns behaviour that gets high reward, but that runs counter to the designers intent \cite{amodei_concrete_2016, dewey2014reinforcement, everitt2016avoiding}.

Inverse reinforcement learning (IRL) was developed in response to difficulties with reward design. In IRL, the goal is to learn a reward function from expert demonstrations \cite{ng2000algorithms, ramachandran2007bayesian, abbeel2004apprenticeship, ziebart2008maximum, neu2009training}. This can be useful when a desired behaviour is easy to demonstrate but difficult to design a reward function for. However, since multiple reward functions can often explain the observed behaviour, the reward function lacks interpretability and is inherently ambiguous \cite{metelli2023towards}.

Reinforcement learning from human feedback (RLHF) instead learns a reward model from human feedback \cite{christiano_deep_2017, ziegler2019fine, bai_training_2022}. This approach is especially useful when aligning agents to human preferences as the agent can optimize for getting good feedback. There are three main parts of RLHF: Feedback collection where humans provide feedback, reward modelling where the feedback is turned into a reward model, and policy optimization where the reward model is used to train a policy/agent with reinforcement learning \cite{casper_open_nodate}.

Our approach bridges the gap between RL and HCI by combining RLHF techniques with user-friendly interfaces and reflective dialogue, making the process of aligning AI agents with individual values more accessible to non-expert users.

\subsection{Preference Elicitation and Active Learning}
When using language feedback for RLHF, it is natural to implement dialogue-based preference elicitation as the mechanism for collecting feedback. In dialogue-based preference elicitation, the goal is to understand a user's preferences through the use of dialogue \cite{priyogi_preference_2019, radlinski_coached_2019}. There are two main approaches to preference elicitation: item-based preference elicitation, where the user is asked about their preferences regarding specific things \cite{adomavicius2005toward, sarwar2001item, loepp2014choice, christakopoulou2016towards, graus2015improving} and feature-based preference elicitation where the user is asked about general features or attributes \cite{llorente2011increasing, sun2018conversational, viappiani2006preference}. Some methods use both item- and feature-based methods \cite{biyik2023preference}, similar to our approach. However, previous work has focused on content recommendation, not agent alignment.

When performing item-based preference elicitation, we must select items to query the user about. Active learning is a subfield of machine learning where the learner is responsible for choosing which examples to request labels for \cite{settles2009active, ren2021survey}. Being selective about which examples to query the user about is important in cases where labels are expensive to obtain \cite{olsson2009literature}. There are generally three strategies for sampling items to query the user about, namely random-, diversity-, and uncertainty-based sampling \cite{monarch2021human}. Random sampling selects items arbitrarily, while diversity-based sampling chooses items that are most different from each other. Uncertainty-based sampling, in contrast, focuses on items the model is least confident about~\cite{mosqueira-rey_human---loop_2023}.

Our system integrates these approaches into an interactive dialogue framework, combining item- and feature-based preference elicitation with active learning and reflective dialogue to capture individual value definitions efficiently.

























% \subsection{Reinforcement Learning and Its Variants}
% Reinforcement Learning (RL) is a branch of machine learning in which an agent learns a policy, i.e., a strategy for selecting actions in an environment, to maximize the rewards it receives. Traditionally, the agent designer crafts a {\it reward function} that is intended to incentivize desirable behaviour and penalize undesirable behaviour, as defined by the designer. However, reward design is notoriously challenging and can result in reward hacking where an agent learns behaviour that gets high reward, but that runs counter to the designers intent \cite{amodei_concrete_2016, dewey2014reinforcement, everitt2016avoiding}.

% Inverse reinforcement learning (IRL) was developed in response to difficulties with reward design. In IRL, the goal is to \textit{learn} a reward function from expert demonstrations \cite{ng2000algorithms, ramachandran2007bayesian, abbeel2004apprenticeship, ziebart2008maximum, neu2009training}. This can be useful when a desired behaviour is easy to demonstrate but difficult to design a reward function for. However, since multiple reward functions can often explain the observed behaviour, the reward function lacks interpretability and is inherently ambiguous \cite{metelli2023towards}. Recently, Kwon et al. \cite{kwon2022reward} proposed a pipeline that relies on a large language model's ability to learn from in-context examples without having to train a reward function from demonstrations.

% Reinforcement learning from human feedback (RLHF) instead learns a reward model from human feedback \cite{christiano_deep_2017, ziegler2019fine, bai_training_2022} instead of expert demonstrations. This approach is especially useful when attempting to align agents to human preferences as the agent can optimize for getting \textit{good} feedback. There are three main parts of RLHF: Feedback collection where humans provide feedback, reward modelling where the feedback is turned into a reward model, and policy optimization where the reward model is used to train a policy/agent with reinforcement learning \cite{casper_open_nodate}. The most common RLHF methodology uses binary preference data obtained through pairwise comparison feedback \cite{christiano_deep_2017}, however, more recently, language feedback has been used as well \cite{bai_constitutional_2022, kwon2022reward, scheurer2022training, chen2023improving}.

% \todo{mention collective feedback aggregation, personalization, virtual democracy}


% \subsection{Preference Elicitation and Active Learning}

% When using language feedback for RLHF, it is natural to implement dialogue-based preference elicitation as the mechanism for collecting feedback. In dialogue-based preference elicitation, the goal is to understand a user's preferences through the use of dialogue \cite{priyogi_preference_2019, radlinski_coached_2019}. There are two main approaches to preference elicitation: item-based preference elicitation, where the user is asked about their preferences regarding specific things \cite{adomavicius2005toward, sarwar2001item, loepp2014choice, christakopoulou2016towards, graus2015improving} and feature-based preference elicitation where the user is asked about general features or attributes \cite{llorente2011increasing, sun2018conversational, viappiani2006preference}. Some methods use both item- and feature-based methods \cite{biyik2023preference}, similar to our approach. Recently, large language models have been used for dialogue-based preference elicitation as well \cite{li2023eliciting, jeong2023factual}. However, previous work has focused on content recommendation, not agent alignment. 

% When performing item-based preference elicitation, we must select items to query the user about. Active learning is a subfield of machine learning where the learner is responsible for choosing which examples to request labels for \cite{settles2009active, ren2021survey}. Being selective about which examples to query the user about is important in cases where labels are expensive to obtain \cite{olsson2009literature}. For example, in our case, we must ask the user to label and explain each trajectory they see, which is time-consuming. There are generally three strategies for sampling items to query the user about, namely random-, diversity-, and uncertainty-based sampling \cite{monarch2021human}. Random-based sampling randomly selects items to query the user about, diversity-based sampling aims to select samples that differ from one another to get information about more parts of the input space, and uncertainty-based sampling seeks to select items that the learner has low confidence about.

% \subsection{Values, Fuzzy Decisions \& the Utility of Reflection}

% Values are principles that guide human behaviour and ethical judgments \cite{schwartz1992universals}. Friedman et al. describe values as ``what a person or group of people consider important in life'' \cite{friedman2013value}. In the context of AI systems, values can manifest in various ways. For example, in a household setting, the value of respect might manifest as an AI assistant using appropriate language or maintaining privacy. In the context of autonomous vehicles, values might include prioritizing passenger safety while also considering the welfare of pedestrians and other road users. Importantly, values vary across cultures, individuals, and contexts \cite{le2009values}. Moreover, while values themselves may be clearly stated, their interpretation and application often become fuzzy when considered in specific contexts \cite{van2013translating}.

% Translating these possibly fuzzy human values into computational terms for AI systems is challenging \cite{russell2019human}. Users may struggle to articulate their values or determine which AI behaviours align with their intent. For example, determining the right balance between passenger safety and broader traffic considerations for an autonomous vehicle involves complex value judgments. The concept of fuzzy preferences \cite{bellman1970decision, ribeiro1996fuzzy} provides insight into this challenge. Fuzzy decision-making acknowledges that preferences, attributes, and objectives in decision processes can be imprecise. In AI alignment, this fuzziness manifests in the difficulty of precisely defining and measuring value alignment. Users may not have clear, a priori knowledge of what constitutes aligned behaviour, and the importance of different behavioural features may be unclear or change based on context.

% Reflection has several notable benefits that can help users clarify their understanding of their preferences and values. For example, it has been found that prompting medical practitioners to reflect can increase diagnostic accuracy~\cite{costa2019effects, fernandes2021adding, mamede2008effects}. Moreover, in consumer research, it has been found that prompting consumers to engage in preference self-reflection can lead to more accurate reporting of preferences and that engaging consumers in realistic decisions can increase preference elicitation accuracy~\cite{hauser2014self}. As our system is concerned with gaining an accurate account of users' values definitions, these findings on reflection are of particular relevance.

% \subsection{Designing for Reflection}

% Designing for reflection has been of interest to HCI researchers for some time \cite{price2003new, yukawa2003co, rogers2006framework, lindstrom2006affective, ghajargar2018designing}. However, Fleck \& Fitzpatrick note that ``designing for reflection'' can mean different things to different researchers~\cite{fleck2010reflecting}. Accordingly, they propose a framework that can be used to think about designing for reflection that includes definitions of various levels of reflection and techniques for supporting reflection. They define level zero of reflection as simply revisiting past events. Level one is defined as revisiting with explanation, where the one reflecting explains and rationalizes events. Level two is dialogic reflection, where relationships in the information and differing perspectives are considered. Level three reflection is transformative, where the reflection prompts a change in one's actions. Level four of reflection is critical reflection, which involves considering wider contexts such as social or moral considerations. Each level of reflection they define is accompanied by various techniques that can prompt users to engage in that level of reflection. 

% The recent rise of LLMs and their chat interfaces presents the opportunity for more tailored and dynamic dialogue to engage users in reflection. However, there has been relatively little work exploring this. Some work has explored the use of LLMs for generating reflective prompts in a design template~\cite{yin_jamplate_2024}, while others have used language prompts to engage users in reflection through single questions or sentence starters~\cite{fessl2017known, renner2016effects, williams2016revising, ifenthaler2012determining}. Further extensions of this approach have included the use of pre-scripted, multi-message dialogues to facilitate a guided reflective process~\cite{kocielnik2018reflection, wolfbauer2022script}.  However, to the best of our knowledge, there has been no work, aside from ours, on integrating LLMs into reflective, back-and-forth dialogue with a user for the purpose of clarifying value definitions.

==> versions/v2.sep.10/3_1_algorithm.tex <==

\RestyleAlgo{ruled}
\begin{algorithm}[!h]
\small
\DontPrintSemicolon
\caption{\systemname{} }
\label{alg:IRDA}

\KwData{
Desired behaviour \texttt{lang(behaviour)}, number of diversity-based trajectories to query the user about $k$, confidence threshold $\epsilon$
}
% \KwResult{Personalized reward model}

\SetKwBlock{Begin}{function}{end function}
% \Begin(){
    Diversity-based sampling of \( k \) trajectories using k-means\;
    \For{\(i \) in \( k \)}{
        Show video of trajectory $i$\;
        Collect user feedback\;
        Add ASCII encoding of trajectory and user feedback to reward model\;
    }
    Generate user feature hypothesis and alternative features\;
    Collect user reflection\;
    Add hypothesis, alternative features, and user reflection to the reward model.
    
    \If{\text{user chooses to enter the preference clarification loop}}{
        return to step 2\;
    }
    \While{model confidence $< \epsilon$}{
        Use uncertainty sampling to select trajectory\;
        Show video of trajectory\;
        Collect user feedback\;
        Add ASCII encoding of trajectory and feedback to reward model\;
        Recalculate \textit{model confidence}   
    }
    \KwRet{Reward model}
% }
\end{algorithm}


% \begin{figure*}[!t]
%     \centering
%     \resizebox{0.75\textwidth}{!}{
%     \begin{tikzpicture}[
%      %start chain = going right,
%     every node/.append style={font=\tiny},
%     startstop/.style = {rectangle, rounded corners,text centered, draw=black},
%     startstop_vertical/.style = {rectangle, rounded corners,text centered, draw=black,rotate=90,anchor=north},
%   block/.style = {draw, align=center,text width=1.5cm},
%   block_vertical/.style = {draw, align=center,text width=1.5cm,rotate=90,anchor=north},
%   line/.style={-latex},
%   dotted_block/.style={draw=black!10!white, rectangle, rounded corners},
% block_vertical_dash/.style={text width=1.5cm,  align=center, draw, dash pattern=on 2pt off 2pt, rectangle,rotate=90,anchor=north}
%                     ]
%     \begin{scope}
% \node (s1) [startstop_vertical] {Start};
% \node (i1) [block_vertical,below of = s1, node distance = 9mm]  {Consent};
% \node (i2) [block_vertical, below of = i1, node distance = 6mm]  {Instructions};

% \node (sb1) [block_vertical, below of = i2, node distance = 15mm]  {Condition 1 \\ ... \\ Condition $m$ };
% %\node (sb1) [block_vertical, below left= 10mm and -1mm of i1]  {condition 1 \\ ... \\ condition $m$ };
% \node at (sb1.east) [below, inner sep=0.5mm]  {Block 1};
% \node (q1) [block_vertical_dash, below of = sb1, node distance = 7mm]  {Question(s)};
% \node (sb2) [block_vertical, below of = q1]  {Condition 1 \\ ... \\ Condition $m$ };
% \node at (sb2.east) [below, inner sep=0.5mm]  {2};
% \node (q2) [block_vertical_dash, below of = sb2, node distance = 7mm]  {Question(s)};
% \node (sbi) [align=center, right of = q2, node distance = 8mm]  {...};
% \node (sb3) [block_vertical, below of = sbi, node distance = 10mm]  {Condition 1 \\ ... \\ Condition $m$ };
% \node at (sb3.east) [below, inner sep=0.5mm]  {$2n-1$};
% \node (q3) [block_vertical_dash, below of = sb3, node distance = 7mm]  {Question(s)};
% \node (sb4) [block_vertical, below of = q3]  {Condition 1 \\ ... \\ Condition $m$ };
% \node at (sb4.east) [below, inner sep=0.5mm]  {$2n$};
% \node (q4) [block_vertical_dash, below of = sb4, node distance = 7mm]  {Question(s)};
% \node (q5) [block_vertical_dash, below of = q4]  {Question(s)};

% \node(measure1)[inner ysep=1mm,inner xsep=1mm,fit=(sb1)(q1)]{};
% \node at (measure1.north) [above, inner sep=0mm]  {Measurement 1};
% \node(measure2)[inner ysep=1mm,inner xsep=1mm,fit=(sb2)(q2)]{};
% \node at (measure2.north) [above, inner sep=0mm]  {Measurement 2};
% \node(measure3)[inner ysep=1mm,inner xsep=1mm,fit=(sb3)(q3)]{};
% \node at (measure3.north) [above, inner sep=0mm]  {Measurement 1};
% \node(measure4)[inner ysep=1mm,inner xsep=1mm,fit=(sb4)(q4)]{};
% \node at (measure4.north) [above, inner sep=0mm]  {Measurement 2};


% \node(rep1)[dotted_block, inner ysep=1mm,inner xsep=1mm,fit=(sb1)(q2)]{};
% \node at (rep1.south) [below, inner sep=0mm]  {Repetition 1};
% \node(rep2)[dotted_block, inner ysep=1mm,inner xsep=1mm,fit=(sb3)(q4)]{};
% \node at (rep2.south) [below, inner sep=0mm]  {Repetition n};

% \node(block1)[dotted_block, inner ysep=4mm,inner xsep=2mm,fit=(i1)(i2)]{};  
% \node at (block1.south) [above, inner ysep=0mm]  {Introduction};
% \node(block2)[dotted_block, inner ysep=3mm,inner xsep=2mm,fit=(rep1)(q5)]{};  
% \node at (block2.south) [above, inner sep=0mm]  {Study};

% \node (e1) [startstop_vertical, below of = q5, node distance = 8mm] {End};

% \draw[->](s1) -- (block1);
% \draw[->](i1) -- (i2);
% \draw[->](rep1) -- (sbi);
% \draw[->](q1) -- (sb2);
% \draw[->](sbi) -- (rep2);
% \draw[->](q3) -- (sb4);
% \draw[->](rep2) -- (q5);
% \draw[->](block1) -- (block2);
% \draw[->](block2) -- (e1);
% %\draw[->,rounded corners](block2.east) -- ++(0.2,0)|-(e1.east);
%     \end{scope}
%     \end{tikzpicture}
%     }
%     \caption{Workflow for the five studies. Dashed blocks are optional question(s) asked depending on each study design. Measurements 1 and 2 are arousal or valence depending on the counter-balanced order.}
%     \label{fig:workflow}
%     \vspace{-1em}
% \end{figure*}







% \begin{figure*}[!t]
%     \centering
%     \resizebox{0.75\textwidth}{!}{
%     \begin{tikzpicture}[
%     node distance=2cm and 0.5cm,
%     auto,
%     block/.style={rectangle, draw, fill=white, text width=5em, text centered, minimum height=15mm, node distance=10em},
%     line/.style={draw, -latex},
%     container/.style={rectangle, draw, dashed, inner sep=1em}
%     ]
    
%     % Nodes
%     \node [block] (stage1) {Stage 1};
%     \node [block, right=of stage1] (stage2) {Stage 2};
%     \node [block, right=of stage2] (stage3) {Stage 3};
    
%     \node [block, right=of stage3, node distance=15em] (reward) {Language-Based\\Reward Modelling};
%     \node [block, right=of reward, node distance=20em] (policy) {Policy Optimization};
    
%     % Container for stages
%     \node [container, fit=(stage1) (stage2) (stage3), label=above:Dialogue-Based Preference Elicitation] (container1) {};
    
%     % Arrows
%     \draw [line] (container1) -- (reward);
%     \draw [line] (reward) -- (policy);
    
%     % Labels
%     \node at (container1.north) [above, inner sep=1mm] {Interactive-Reflective Dialogue Alignment};
    
%     \end{tikzpicture}
%     }
%     \caption{Workflow depicting the stages of Interactive-Reflective Dialogue Alignment leading to Policy Optimization.}
%     \label{fig:workflow}
% \end{figure*}



% % \begin{algorithm}[]
% % \DontPrintSemicolon
% % \caption{Instruction Collection Algorithm}
% % \KwResult{Collect user feedback and refine system hypothesis.}

% % \SetKwBlock{Begin}{function}{end function}
% % \Begin(InstructionCollection){
% %     Diversity based sampling of \( k \) trajectories\;
% %     \For{\(i \) in \( k \)}{
% %         Show video\;
% %         Collect feedback\;
% %     }
% %     Collect user reflection\;
% %     \If{refusal}{
% %         Go back to initial loop\;
% %         \For{\(i \) in \( k \)}{
% %             Show video\;
% %             Collect feedback\;
% %         }
% %     }
% %     Uncertainty based sampling of \( j \) trajectories\;
% %     \For{\(i \) in \( j \)}{
% %         Show video\;
% %         Collect feedback\;
% %     }
% % }
% % \end{algorithm}

==> versions/v2.sep.10/3_system.tex <==
\section{Interactive-Reflective Dialogue Alignment (IRDA) System}

\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{figures/rlhf_flow_chart.pdf}
  \caption{Overview of the RLHF pipeline with \systemname{}.}
  \Description{The diagram outlines a sequential process, titled "Interactive-Reflective Dialogue Alignment," in a dashed box divided into two main components: 'Feedback Collection' and 'Reward Modeling.' The 'Feedback Collection' part is subdivided into three stages: Stage 1: Initial Item-Based Preference Elicitation. Stage 2: Feature-Based Preference Elicitation. Stage 3: Uncertainty-Reduction Item-Based Preference Elicitation. Following this is the 'Reward Modeling' component, which contains 'In-Context Language-Based Reward Modeling.' The final block, outside of the dashed area, is 'Policy Optimization.'}
\end{figure*}

We introduce an interactive system, named \systemname{} (IRDA), which aims to enable end users with no particular expertise in machine learning to define agent behaviour that is aligned with their subjective definitions of a human value and generate a reward model that can be used to train an agent based on this definition. The system consists of three components: a user-facing \textbf{chat interface} (shown in Figure~\ref{system_screenshot}), which allows the user to interact with the system; a \textbf{value elicitation module}, which generates dialogue to engage users in a reflective conversation aimed at helping users articulate their own definition of a value, and a \textbf{reward modelling module} which uses the information gained in conversation with the user to create a language-based reward model.

Together, these components form a system that facilitates the first two stages of RLHF, namely feedback collection and reward modelling. In particular, the chat interface and the value elicitation module facilitate feedback collection, and the reward modelling module facilitates reward modelling. The third stage of RLHF is policy optimization, where an agent is trained using the reward model to adopt behaviours that are aligned with the user-defined value. Policy optimization is not part of our system and is outside the scope of this paper, but the reward models generated by our system are compatible with nearly all policy optimization methods.

We will begin by outlining our design aims, then we will provide a high-level overview of the system and then describe each component in more detail.

\subsection{Design Aims}
Our system is intended for the end-users of AI agents, and we do not assume the users of our system will have any technical expertise. As such, the design aims for our system are centred around the idea of making the system easy and quick to use while maintaining good performance. More specifically, our system for allowing end users to align agents to their unique individual values should have the following properties:
\begin{enumerate}
    \item The system should not require any special technical knowledge (e.g., how to program or how to design a ``good'' reward function).
    \item The system should be sample-efficient (i.e., intelligent in selecting the most informative examples for the user to label).
    \item The system should be able to capture individual differences and unique conceptions of desirable behaviour associated with a value.
\end{enumerate}

\subsection{Multi-Agent Apple Farming Environment}\label{maaf_description}
To better illustrate our system, we will now describe one environment used in our evaluation, the \textit{Multi-Agent Apple Farming Environment}.  In reinforcement learning, agents learn how to behave in an environment by receiving rewards and penalties. In this case, our environment is a 6$\times$6 grid where the agents are rewarded for picking apples and receive no reward for collecting garbage. There is one blue ``main'' agent in the environment and three grey ``background'' agents. Each one of the agents owns one of the four 3$\times$3 quadrants, which each represent an orchard. Each agent is free to move around the whole grid; however, two of the three background agents are programmed to be stationary. The main agent is the agent the user gives feedback about. The environment can be seen in Figure~\ref{fig:teaser}.

\subsection{System and User Flow: An Overview}

Our systems allow users to specify how agents should behave in order to be aligned with a value---for instance, picking apples but being ``respectful'' to neighbours. The user flow and how it is supported by the system is described below (and is shown in algorithmic form in \ref{alg:IRDA} in the appendix).

Upon entering our system, users are presented with a greeting message outlining the purpose of the system as well as a preview of the environment. Users are then asked to briefly explain how they would like the agent to act.
% To begin, we allow the user to specify how they would like the agent to act in natural language. 
For example, a user could say ``I would like the agent to act respectfully.'' 

We assume the agent has not been trained, so we collect a large pool of trajectories (sequences of the agent taking actions in the environment). We then use \textit{diversity-based trajectory sampling}, a technique from active learning, to find $k$ trajectories where the agent behaves in diverse ways. The goal of diversity-based sampling, in this case, is to find trajectories where the agent acts according to the user's instruction and where it does not. The system then shows the user these $k$ trajectories, one at a time, and asks the user to explain if the agent is acting according to their value definition.

Based on the way the user assesses each trajectory, the system forms a hypothesis regarding the behavioural features (see Section \ref{section:s1_features} and Section \ref{section:s2_features} for examples of behavioural features) on which the user bases their decisions (see the ``Labelling Hypothesis'' box in \autoref{fig:teaser} for an example hypothesis). The system also proposes additional features that could be relevant to the user (see the ``Alternative Perspectives'' box in \autoref{fig:teaser}). The user is then prompted to reflect on whether the hypothesis is correct and why or why not the additional features proposed are relevant to their desired agent behaviour. If the user agrees with one of the additional features proposed by the system or has changed their mind in another way as a result of this reflective step, they can enter into the \textit{preference clarification loop} and re-explain the $k$ trajectories they initially saw with their new perspective.

All of the information collected from the user is then used to build a temporary language-based reward model. The temporary reward model assigns binary rewards---0 if the user would not approve of the agent's behaviour and 1 if the user would approve of the agent's behaviour---to a small pool of trajectories that it selects via \textit{uncertainty-based sampling}~\cite{mosqueira-rey_human---loop_2023}. The trajectory where the model is least certain about the reward to assign is then shown to the user, and the user is asked to explain whether the agent behaves as they would like it to. A minimum certainty threshold, $\epsilon$, can be set, and this uncertainty reduction process can be repeated until the model is at least as certain as the threshold about every trajectory in the uncertainty pool. We refer to this iterative process as the \textit{uncertainty reduction loop}. Each time the user explains one of the trajectories the model is uncertain about, this information is added to the reward model, thus making it less uncertain about similar trajectories.

Ultimately, all of the information gained from the user is combined into a language-based reward model that can effectively administer rewards to an agent when it acts in accordance with the user's value definitions. Depending on the complexity of the desired behaviour and environment, this reward model can then be used to either train a more efficient reward model or to train an agent directly.

We will now describe the system in more detail, starting with how the system collects feedback from the user, followed by how the system uses the feedback to create a reward model.

\subsection{Feedback Collection} \label{feedback_collection}

Our system works with the user to refine their value definition and understand agent behaviours that align with that definition. In the spirit of making our system accessible to users with varying backgrounds and skill sets, we collect feedback from users in natural language through a chat interface shown in Figure~\ref{system_screenshot}.
% In addition to being a common and accessible mode of interaction, 
Dialogue is an engaging mode of interaction~\cite{ruan2019quizbot, wolfbauer_script_2022}, making it an appealing feedback collection method. We frame our language-based feedback collection as \textit{dialogue-based preference elicitation}, where we collect feedback about users' preferences regarding the agent's behaviour. The dialogue is generated by the \textbf{value elicitation module}.

\subsubsection{Dialogue-Based Preference Elicitation}\label{dialogue-based_preference_elicitation}
We employ both item-based and feature-based preference elicitation in multiple stages outlined below. The dialogue-based preference elicitation process is shown in Figure \ref{fig:teaser}. 

\begin{figure}[htbp]
    \centering
    \begin{minipage}{0.4\textwidth}
    \begin{lstlisting}
----- Step: 0 -----
The main agent (M) is in the 
quadrant (orchard) that it owns.
 M   .   . | .   G   .
 A   .   . | G   .   .
 .   .   . | .  AA   B
-----------------------
 .   .   . | .   .   .
 B   .   A | B   .   .
 A   .   . | A   A   .
=========================
----- Step: 1 -----
Main agent moved from [0, 0] to [1, 0]. 
 .   M   . | .   G   .
 A   .   . | G   .   .
 .   .   . | .  AA   B
-----------------------
 .   .   . | .   .   .
 B   .   A | B   .   .
 A   .   . | A   A   .
    \end{lstlisting}
    \end{minipage}
    \caption{ASCII encoding of two timesteps of a trajectory of the multi-agent apple farming environment.}
    \label{fig:ascii-encoding}
\end{figure}

\subsubsection*{Stage 1: Initial Item-Based Preference Elicitation.} To perform item-based preference elicitation, we first select items (specific examples of agent behaviour) to query the user about. 

At the start of the interaction with the user, we lack information about the user's preferences, and thus, we employ \textit{diversity-based sampling} to find a set of trajectories where the agent exhibits a diverse set of behaviours in varying situations. To do this, we begin by sampling a large pool of over 1000 trajectories. We turn each trajectory into a numerical array that gives a full representation of the state of the environment at each time step. For example, in a 30-step trajectory in the multi-agent apple farming environment, we can encode each step as multiple arrays of the same shape as the grid. In each array, for a step, we can encode the position of a certain type of entity within the environment. The numerical encoding for a single timestep is shown in Figure~\ref{numerical_encoding}.


\begin{figure}
  \centering
  \includegraphics[width=0.5\linewidth]{figures/env_to_array.png}
  \caption{A numerical encoding of one timestep of the multi-agent apple farming environment. Agent positions are encoded in one array, apple positions in a second array, and garbage positions in a third.
  }
  \Description{}
  \label{numerical_encoding}
\end{figure}


With the pool of numerically encoded trajectories in hand, we perform $k$-means clustering to split the trajectories into $k$ distinct clusters. Since we want to query the user about a diverse set of trajectories in this initial phase, we select one trajectory from each of the $k$ clusters. In particular, for each group, we select the trajectory closest to the arithmetic mean, or the centroid, of all the trajectories in the cluster.

The system asks the user to explain whether the agent is aligned with their preferences in each of the $k$ trajectories, one at a time, using 1-3 sentences. For instance, if a user were trying to train an agent to behave respectfully, the system would ask, ``\texttt{Does the agent act respectfully? Please explain your reasoning using 1-3 sentences.}''

\subsubsection*{Stage 2: Feature-Based Preference Elicitation.}

% \carter{Possibly explain trajectory encoding here?}
Once we have collected information from the user about each of the $k$ trajectories selected through diversity-based sampling, we use a large language model (GPT-4 Turbo) to make a hypothesis about what features the user is basing their decisions on and other features the user could consider. To do so, we parse each trajectory into an ASCII representation (see Figure \ref{fig:ascii-encoding} for an example) and pass this along with the user's explanation to the LLM. In the prompt, we ask the LLM to make a hypothesis about what features the user is basing their decisions on and to offer alternative features the user could consider.

For example, in the multi-agent apple farming environment, where an agent owns one of four orchards in the environment, the user may base their definition of ``respectful'' behaviour on whether the agent stays in its own orchard. A simplified example of a response from the system could be:
\begin{quote}
    \texttt{Based on your explanations, it seems as though a key factor in determining whether the agent's behaviour is respectful or not is whether the agent stays in its own orchard.}
    \texttt{You could also consider:}
    \texttt{
    \begin{enumerate}
        \item Whether the agent helps pick up garbage
        \item Whether the agent steals apples from other agents
    \end{enumerate}
    }
\end{quote}

The user is then prompted to explain if the hypothesis the system made is correct and if the other features should be considered. This step is important for a number of reasons. First, understanding the features on which the user bases their decisions allows for improved generalization of the reward model. The system can use these features, or patterns of behaviour, as decision criteria when assessing whether the agent's behaviour in a trajectory aligns with the user's intent. Second, this step encourages the user to reflect on their definition and consider alternative perspectives. This reflection can assist users in gaining a clearer understanding of the specific behaviour they want the agent to demonstrate. Third, if the diversity-based sampling in the initial item-based preference elicitation phase does not select any trajectories where a certain behavioural feature is present that would be important to the user, the alternative or additional features proposed by the system can help uncover these. This can help the system gain a more holistic understanding of the user's preferences, even when only querying the user about a handful of items.

If the user updates the features they think are important based on the system's proposed alternatives, they can optionally re-explain the initial $k$ trajectories. We refer to this as the \textit{preference clarification loop} as it allows users to iteratively reflect on what features or behavioural patterns they would like the agent to embody. This loop simultaneously helps the user better understand their own preferences and helps the system gain a clearer understanding of the user's true intent. 

\subsubsection*{Stage 3: Uncertainty-Reduction Item-Based Preference Elicitation.}
Once the user has exited the preference clarification loop, the system creates a \textit{temporary} reward model based on the user's expressed intent. The reward model can be thought of as a classifier - the input is an ASCII representation of a trajectory, and the output should be a 1 if the agent's behaviour aligns with the user's expressed intent and 0 otherwise. The reward model will be covered in more detail in Section \ref{reward_modeling}.

The reward model is used to assign rewards to a pool of trajectories. Since our reward model is based on an autoregressive transformer (LLM), we can find trajectories where the reward model had high uncertainty about what the reward should be by comparing the token probabilities for a positive classification (reward) or a negative classification (no reward). For example, if the user is training the agent to be respectful, we compare the probability of the reward model outputting the "respectful" token to the probability of the model outputting the "disrespectful" token. If the probabilities are close to one another, then the model is less certain, and if they are very different (e.g. 0.99 and 0.01), then the model has high certainty about whether the agent acts according to the user's intent. The "confidence" of the model can be thought of as the absolute value of the difference between the two token probabilities. We collect feedback from the user about the trajectory where the model had the lowest confidence. Each time we query the user to explain a trajectory for which the model had low certainty, we add the ASCII representation of the trajectory and the user's explanation to the reward model to increase its confidence in similar situations. We can set a minimum confidence threshold and continue to do this until the model's confidence about each trajectory in the uncertainty pool is above the threshold. This is referred to as the \textit{uncertainty reduction loop} as it iteratively reduces the model's uncertainty about the user's value definition.
  
\subsubsection{Reflective Dialogue}

To help the user understand the behaviour they would like the agent to embody and convey a clearer picture to the system, we designed our dialogue to engage the user in reflective, system 2 thinking \cite{evans2019reflections}. Work on dual process theory has found that intuitive (system 1) and reflective (system 2) thinking may not be completely distinct and, rather, that both systems may cooperate in reasoning and moral reasoning \cite{evans2019reflections, cecchini2021dual}. In particular, it has recently been proposed that reflective system 2 thinking can help one justify, rationalize and explain their intuitions. This insight is important for dialogue-based preference elicitation. \textbf{A user may have an intuitive, fuzzy understanding of how they want the agent to act, but for the system to capture this, the user must be able to explain and justify this clearly.} As such, we draw upon insights from HCI research on "designing for reflection"~\cite{fleck2010reflecting} to help the user reflect on and explain their intent to the system.

In particular, we draw on Fleck and Fitzpatrick's levels of reflection and implement techniques they suggest can support reflection, such as asking reflective questions and providing alternative perspectives~\cite{fleck2010reflecting}.

During both stages of item-based preference elicitation (see Stage 1 \& Stage 3 in Section~\ref{dialogue-based_preference_elicitation}), we designed the system dialogue to engage the user in level 1 reflection, referred to as ``reflective description.'' The system asks the user to state whether the agent acts in the way they desire and to justify and explain their decision. This allows the user to reflect on the reasoning behind their decision and also gives the system more information about the user's intent and preferences. When the user provides a decision and an explanation, the explanation can help the reward model generalize to other situations as it elucidates the features the user is using to make their decisions\cite{lampinen-etal-2022-language, kwon2022reward}.

\begin{figure}
  \centering
  \includegraphics[width=0.5\linewidth]{figures/system_screenshot.jpeg}
  \caption{System screenshot showing the user-facing chat interface of the \systemname{} system.
  }
  \Description{}
  \label{system_screenshot}
\end{figure}

During the feature-based preference elicitation stage (see Stage 2 in Section \ref{dialogue-based_preference_elicitation}), the system engages the user in level 2 reflection, referred to by Fleck and Fitzpatrick as ``dialogic reflection'' which ``primarily involves seeing things from a different perspective'' \cite[p.~218]{fleck2010reflecting}.

% To achieve this, we prompt an LLM to make a hypothesis about what features the user is basing their decisions on and to propose alternative features the user could consider. This is then shown to the user, and they are prompted to explain if the hypothesis is correct and why or why not the other features should be considered. Again, in doing this, the user clarifies their own understanding of the behaviour they would like the agent to embody and communicates this to the system.

Overall, the goal of the reflective dialogue is twofold. First, it helps the user clarify their own, possibly fuzzy, preferences. And second, it helps the system understand the user's preferences and intent. 


\subsection{Reward Modelling} \label{reward_modeling}
Once the feedback from the user has been collected, the next step in the RLHF pipeline is to create a reward model that can give feedback to the learning agent on behalf of the human. The creation of the reward model is handled by the \textbf{reward modelling module}. Creating a reward model that can issue rewards on behalf of humans is important as, depending on the complexity of the environment and the desired behaviour, it can take millions~\cite{pardo2018time} or even billions~\cite{agapiou2022melting} of timesteps for an agent to learn the desired behaviour. The reward model can act on behalf of the user, thus relieving the user of giving feedback during agent training.
 

\subsubsection{In-Context Language-Based Reward Model}

% The reward model can be thought of as a classifier in that it receives a trajectory parsed into ASCII (see \autoref{fig:ascii-encoding}) as input and outputs $1$ if the agent's behaviour aligns with the user's expressed intent and $0$ otherwise. To achieve this, we provide an LLM with the information collected about the user during the dialogue-based preference elicitation and ask the LLM whether the agent's behaviour in the input trajectory is aligned with the user's expressed intent. If the LLM thinks the agent behaves according to the user's expressed intent, we parse this to a 1 and otherwise a 0.

Our reward model functions as a classifier, evaluating agent behaviour based on user-defined values. The model receives as input a trajectory encoded in ASCII format, a process detailed in \todo{Appendix A}. This encoding preserves essential spatial and temporal information while enabling efficient processing by language models (see \autoref{fig:ascii-encoding} for an example).
The model leverages two key elements to classify a trajectory: (1) The encoded trajectory and (2) the user feedback collected during dialogue-based preference elicitation.

Using this information, we prompt the LLM to assess whether the agent's behaviour in the given encoded trajectory aligns with the user's expressed intent. The LLM's output is then parsed into a binary classification: 1 if the behaviour aligns with user intent, 0 otherwise.

To achieve this, we create a prompt that includes 
\begin{enumerate}
    \item a description of the environment and the ASCII characters used in the encoding,
    \item the information gained from the user during the dialogue-based preference elicitation,
    \item a description informing the language model that its goal is to predict whether the agent's behaviour is aligned with the user's intent,
    \item an ASCII representation of the trajectory that the model is to label,
    \item text to encourage the model to engage in chain-of-thought reasoning,
    \item and instructions about how the LLM is to format its response so that the output can be programmatically parsed.
\end{enumerate}

Two major findings about LLM capabilities inspired the design of this prompt. First, LLMs are effective in-context, few-shot learners \cite{brown_language_2020}. This means that a trained LLM, with fixed parameters, can learn new patterns by including the beginning of a pattern as context and asking the model to continue the pattern. In settings similar to ours, this has been shown to be far more sample efficient than traditional supervised learning~\cite{kwon2022reward}. The pattern of interest, in our case, is what behaviour the user deems to be aligned with their intent.
The second finding is that prompting LLMs to engage in chain-of-thought reasoning can greatly increase their performance~\cite{kojima2022large}. The idea is that the model forms an argument first and then, due to the auto-regressive nature of language models, uses the argument it made to determine a final answer. 
% In other words, the LLM must justify its answer before giving it.

Since our LLM-based reward model receives a full trajectory as input and outputs a reward, it can deal with non-Markovian rewards. This means that the reward model can evaluate the agent's behaviour over multiple time steps when determining the reward. We hypothesized that this would be important for capturing users' preferred agent behaviour, and this was supported by our empirical findings discussed in Section \ref{section:s1_discussion}.
% For example, some users thought that it was only respectful for an agent to enter another agent's territory if that other agent had already entered their territory. This is markedly non-Markovian as it cannot be determined in a single timestep.


==> versions/v2.sep.10/4_study_design.tex <==
\section{Study Design \& Methodology}
We evaluated our system, \systemname{} by comparing it to two baselines in two different environments: a multi-agent apple farming environment and the moral machine setting \cite{awad2018moral}. 

Our studies employ a within-subject design, collecting data from each participant to train various language-based reward models, supervised learning baselines, and for a test set to evaluate these methods. This section describes the methodology common to both studies, with specifics provided in their respective sections.

\subsection{Procedure} Participants used our interface to specify how they would like the agent to act via our dialogue-based preference elicitation process. Participants then labelled 50 scenarios and were interviewed.

\textit{Introduction ($\sim$5min)} - After completing the consent form and the demographic questions, the mechanics of the environment were fully explained to the user. We explained the environment mechanics as thoroughly as possible so that differences observed between participants stemmed from their opinions, not hidden assumptions about the environment. 
Following the explanation of the environment, participants were told that they would only be evaluating the blue agent that starts in the upper left quadrant and that they should assess whether this agent acts respectfully according to their own understanding.

\textit{Dialogue} - The participant began by conversing with the system about the agent's behaviour following the dialogue structure presented in section \ref{dialogue-based_preference_elicitation}. To control the amount of time users spent on the activity, we limited the user to one preference clarification loop and one uncertainty reduction loop. 

\textit{Labelling} - Following the participants' dialogue interaction with the system, participants labelled 50 scenarios. Each participant labelled the same scenarios, which allowed us to assess how much the participants agreed on the labels.

\textit{Semi-structured Interview ($\sim$10min)} - After completing the labelling task, each participant was asked whether they felt they were able to give the system a good understanding of their decision-making if they were always able to articulate why they chose a label, if it was ever difficult to decide, and if they thought their labelling behaviour changed over time. The interview aimed to determine two things. First, it sought to find out if people could verbally explain their definition of value. Second, it attempted to discover whether these definitions changed over time and what factors caused any changes.

\subsection{Baseline Comparisons}
We compare our system to another language-based reward modelling pipeline proposed by Kwon et al. \cite{kwon2022reward} to test if our reflective dialogue is useful. Additionally, we compare the language-based methods to various supervised learning methods to test the efficacy of language-based reward modelling.

\subsubsection{Language-Based Baseline}\label{baseline}
Kwon et al. \cite{kwon2022reward} proposed a reward modelling pipeline for text-based environments where the user selects multiple examples from a palette of examples of the agent behaving as they would desire, accompanied by explanations. We slightly modify their pipeline in the following way: Instead of asking the user to select examples from a handcrafted palette, we choose the examples the user sees with the diversity-based sampling procedure described in Stage 1 of Section~\ref{dialogue-based_preference_elicitation}.
As a result, we focus on the utility of the reflective dialogue.

Since the baseline pipeline above is a subprocess of our full system, \systemname{}, the user only interacts with our system. But, when forming the reward model for the baseline, we only include the information collected from the user during the first iteration of Stage 1 of the dialogue-based preference elicitation before they have reflected, mirroring the pipeline proposed in \cite{kwon2022reward}.

\subsubsection{Supervised Learning Baseline}
In addition to language-based reward models, we compared to supervised learning (SL) methods. All SL methods we compared to are neural networks.
For the supervised learning models, we utilized numerical encodings of the examples and labels provided by participants. In study one, the numerical encoding was based on the grid map (see \autoref{numerical_encoding}). For study two, we trained two versions: one used a feature-based description of the scenario, while the other used images of the scenario.
During the labelling phase, each participant annotated 50 scenarios. We reserved 30 scenarios per participant for training the supervised learning models. We developed two types of models: individual models ($M^\text{ind}_i$) and a collective model ($M^\text{col}$). The $M^\text{ind}_i$ models were trained separately for each participant $i$ using only their data, while the $M^\text{col}$ model was trained by aggregating data from all participants.


\subsection{Analysis}

\begin{table}
\centering
\caption{Mapping of Analysis Methods to Research Questions}
\label{tab:analysis-rq-mapping}
\begin{tabular}{>{\raggedright\arraybackslash}p{0.6\textwidth}ccc}
\toprule
\textbf{Analysis Method ($\S$)} & \textbf{RQ1} & \textbf{RQ2} & \textbf{RQ3} \\
\midrule
\rowcolor{lightgray}
Inter-Annotator Agreement (\ref{section:inter_ann_agree}) & $\checkmark$ &  & $\checkmark$ \\
Evaluation of Language-Based Reward Model Performance (\ref{section:eval_lbrm}) &  & $\checkmark$ & \\
\rowcolor{lightgray}
Comparison to Supervised Learning (\ref{section:comp_sl}) & $\checkmark$ &  & $\checkmark$ \\
Qualitative Analysis of Participant Decision Making (\ref{section:qual_decision}) & $\checkmark$ &  &  \\
\rowcolor{lightgray}
Analysis of Feature Similarity Between Participants (\ref{section:feature_similarity})& $\checkmark$ &  & $\checkmark$ \\
Thematic Analysis of Interview Data (\ref{section:thematic})&  & $\checkmark$ & $\checkmark$ \\
\bottomrule
\end{tabular}
\end{table}

Our analysis aims to answer the following three questions:
\begin{enumerate}[label=\textbf{RQ\arabic*:}]
\item Do value definitions significantly vary between participants?
\item Does structured reflection enhance language-based reward modelling?
\item When is individualized language-based reward modelling effective?
\end{enumerate}

To address these questions, we employ a mixed-methods approach, combining quantitative analyses of model performance and inter-annotator agreement with qualitative analyses of participant decision-making processes and experiences. The following subsections detail our analytical methods, each designed to provide insights into one or more of our research questions.

\subsubsection{Inter-Annotator Agreement}\label{section:inter_ann_agree}
We assess the inter-annotator agreement between participants on the test set of scenarios they labelled in each study. Since each participant labelled the same test scenarios, we can use Fleiss' kappa value to quantify the inter-annotator agreement between the participants \cite{landis1977measurement}. Generally, kappa statistics below 0 indicate ``poor'' agreement and kappa statistics above 0.8 indicate ``nearly perfect'' agreement \cite{landis1977measurement}. This analysis directly addresses \textbf{RQ1} by quantifying how much participants agree when labelling examples. Low agreement suggests diverse value definitions, while high agreement indicates more uniform values across participants. It also informs \textbf{RQ3} by indicating when individualized approaches might be more beneficial than collective ones.


\subsubsection{Evaluation of Language-Based Reward Model Performance}\label{section:eval_lbrm}
Our evaluation compares our system's performance against the baseline language-based reward modelling system that does not leverage dialogic (level 3) reflection. We use a performance metric, $P$, calculated for each participant on both systems. We denote $P_i^\text{IRDA}$ and $P_i^\text{baseline}$ as the performance metrics for participant $i$ on our system and the baseline system, respectively. The choice of performance metric varied between studies: the first study used balanced accuracy due to high class imbalance, while the second study used standard accuracy.

For each participant, we generate rewards (labels) for 20 scenarios they previously labelled, using both systems. We then calculate $P$ for each system per participant. This process yields $n$ pairs of $P$ values, where $n$ is the total number of participants.
We conducted three statistical tests on the $P$ values:
\begin{enumerate}
    \item We bootstrapped 95\% confidence intervals for the mean by resampling 10,000 times with replacement.
    \item For each participant, we calculated the difference $\Delta P_i = P_i^\text{IRDA} - P_i^\text{baseline}$ and bootstrapped these differences.
    \item We compared the $P$ values for each system using the Wilcoxon signed-rank test. This non-parametric test was chosen over parametric alternatives as it is less prone to false positives and more robust when the data distribution is unknown or skewed \cite{bridge1999increasing}.
\end{enumerate}

This analysis primarily addresses \textbf{RQ2} by comparing the performance of systems with and without dialogic reflection, allowing us to assess if structured reflection enhances language-based reward modelling.


\subsubsection{Comparison to Supervised Learning}\label{section:comp_sl}

We compared our language-based systems to traditional supervised learning approaches. Both $M^\text{ind}_i$ and $M^\text{col}$ were trained incrementally, gradually increasing the number of samples used per participant. This methodology allowed us to analyze how model performance evolved with increasing data availability.
For each increment, we calculated $P^\text{ind}_i$ and $P^\text{col}_i$ for each participant $i$, representing the performance of the individual and collective models, respectively. To ensure robust statistical analysis, we bootstrapped these values with replacement using 10,000 resamples.

This comparison helps answer \textbf{RQ3} by revealing when language-based methods outperform supervised learning approaches under various conditions. It also indirectly informs \textbf{RQ1} by showing if individualized language-based models consistently capture personal value definitions better than collective supervised models.

\subsubsection{Qualitative Analysis of Participant Decision Making}\label{section:qual_decision}
We conducted a detailed analysis of the message exchanges between participants and the system to gain insight into participants' decision-making processes. We employed an inductive coding approach, systematically reviewing the messages to identify key features and criteria that participants used in their decision-making. Our coding process involved multiple passes through the data, with iterative refinement of the codebook to ensure it captured the full range of decision-making strategies observed.

This analysis directly addresses \textbf{RQ1} by identifying different features and criteria used by participants, providing rich evidence of how value definitions differ.


\subsubsection{Analysis of Feature Similarity Between Participants}\label{section:feature_similarity}
To quantify how similar participants were in their use of decision-making features, we employed the Jaccard similarity coefficient. This measure calculates the overlap between two sets of items which, in our case, are features the two participants used to make decisions~\cite{jaccard1912distribution}. We computed the Jaccard similarity coefficient for every possible pair of participants, using the set of decision-making features each participant employed (as identified in our qualitative analysis). To estimate the overall similarity across our participant pool, we then calculated the mean of these pairwise Jaccard coefficients. To ensure robustness, we used bootstrapping with 10,000 resamples (sampling with replacement) to determine the 95\% confidence interval for this mean Jaccard similarity coefficient. 

This quantitative measure helps answer \textbf{RQ1} by providing a numerical representation of how much participants' decision-making features overlap. Low similarity scores strongly support the notion that value definitions vary significantly between participants. It also informs \textbf{RQ3} by providing a numerical indicator for when collective vs. individualized approaches might be more appropriate.


\subsubsection{Thematic Analysis of Interview Data}\label{section:thematic}
We conducted semi-structured interviews with participants to understand their experiences. The interview transcripts were analyzed using a thematic analysis approach guided by the principles outlined by Braun and Clarke \cite{braun2006using}. We followed a six-phase process: familiarization with the data, generating initial codes, searching for themes, reviewing themes, defining and naming themes, and producing the report.

This analysis addresses \textbf{RQ2} by revealing if reflection enhanced participants' ability to articulate their values, which is crucial for effective language-based reward modelling. It also informs \textbf{RQ3} as language-based reward modelling requires that participants can articulate their value definition to be effective. 


==> versions/v2.sep.10/5_study1.tex <==
\section{Study 1 - Multi-Agent Apple Farming}
Study 1 investigates the utility of our system for learning about participants' definition of \textit{respectful} agent behaviour. The goal is to understand if our system, which uses reflective dialogue, can effectively capture individual definitions of respect and whether individual definitions differ. 

\textit{\textbf{Environment \& Task.}}
% \subsubsection*{Design}
The multi-agent apple farming grid world, described in \autoref{maaf_description}, was used in this study. Participants were asked to evaluate if the agent was acting respectfully. 

% Participants first went through the dialogue phase and then labelled 50 trajectories.
\textit{\textbf{Baselines.}}
We compared our system to another language-based system described in subsection \ref{baseline}. We also compare our system to two types of reward models trained with supervised learning: Individual models, $M^\text{ind}$, and a collective model, $M^\text{col}$. One individual model was incrementally trained for each participant, and one collective model was trained for all participants. These models are MLPs with one hidden layer with 32 neurons, trained with a learning rate of $0.001$ and the Adam optimizer. The input to the models was the numerical encoding shown in \autoref{numerical_encoding}.

\textit{\textbf{Participants.}}
% \subsubsection*{Participants}
We recruited 21 participants from our institution (18 to 39 age range, M=23.86, 7 self-identified as male and 14 as female). When asked to rate their level of familiarity with reinforcement learning on a 5-point Likert ranging from ``very unfamiliar'' (1) to ``very familiar'' (5), the mean level of familiarity was 2.48, with the mode and median being 2. The Likert-scale data is visualized in figure \ref{fig:rl_familiar} and highlights that more than half of participants were ``unfamiliar'' or ``very unfamiliar'' with reinforcement learning.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.5\linewidth]{figures/rl_familiar_s1.png}
  \caption{Participant familiarity with reinforcement learning in Study 1.}
  \Description{}
  \label{fig:rl_familiar}
\end{figure}

% \textit{\textbf{Grid World Environment: }}






% To answer the second question, we measure how much the reward models produced by each pipeline agree with the participants they are modelling. We then compare this to how much the participants agree with one another. Specifically, we created two reward models for each participant: one using the baseline pipeline and another using our pipeline (as described in section \ref{partic_reward_modelling}). We assess the agreement between each participant's responses and their corresponding reward models using the Fleiss' kappa metric. By averaging these agreement scores across all participants for both pipelines, we obtain a measure of how well the reward models from each pipeline match the participants' views. We also bootstrap the agreement scores to obtain confidence intervals for the average agreement between the participants and the reward models from each pipeline. We then calculate the inter-annotator agreement between all participants again using Fleiss' kappa. \todo{add citation and explanation for the choice of Fleiss' kappa. Maybe add a word of warning?}

\subsection{S1 -- Quantitative Results}

On average, participants took 15 minutes 57 seconds (SD $=$ 6 min. 43 sec., range: 6 min. 59 sec. - 30 min. 55 sec.) to complete the dialogue with the system and 13 minutes 37 seconds (SD $=$ 3 min. 2 sec., range: 6 min. 55 sec. - 18 min. 26 sec.) to complete the labelling of 50 trajectories. Of 21 participants, 7 (33.$\bar{33}\%$) entered the \textit{preference clarification loop} for one iteration.

\subsubsection{S1 - Inter-Annotator Agreement}
We observed a Fleiss' kappa value between all participants' labels on the 50 labelled trajectories of $\kappa = 0.336$, indicating ``fair'' agreement among participants \cite{landis1977measurement}. The Fleiss' kappa statistic of 0.336 we observed lends credence to the idea that human values and preferences are subjective and personal.

\subsubsection{S1 -- Evaluation of Language-Based Reward Model Performance.}
On average, the reward models produced by our pipeline received significantly higher balanced accuracy scores (measured in percentages) than the baseline system by 9\% (95\% CI: [5\%, 13\%], M = $68\%$ vs. M = $59\%$, p=.002). The distributions of the balanced accuracies for each pipeline are visualized in Figure~\ref{accuracy_dist_s1}. The distribution of the per participant difference in balanced accuracy is shown in \autoref{accuracy_diff_s1}.



% The average Fleiss' kappa statistic for the reward models generated with the baseline system and the participants was $\kappa = 0.25$ (95\% CI:[0.14, 0.35]), indicating. The average Fleiss' kappa for the reward models generated with our pipeline and the participants was $\kappa = 0.36$ (95\% CI:[0.28, 0.43]).

% This result indicates that the reward models produced by our pipeline, using \systemname{}, on average, agree more with each participant than the participants agree with each other about what agent behaviour is respectful. \carter{However, this result should be taken with caution?}

\begin{figure}
  \centering
  \includegraphics[width=0.5\linewidth]{figures/balanced_accuracy_s1.png}
  \caption{Distributions of the balanced accuracies of the language-based reward models generated with our pipeline (IRDA) compared to those of the language-based reward model generated with the baseline pipeline in Study 1.}
  \Description{}
  \label{accuracy_dist_s1}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=0.5\linewidth]{figures/balanced_accuracy_diff_s1.png}
  \caption{Distribution of the per participant difference in balanced accuracy between the language-based reward model generated with our pipeline (IRDA) compared to the language-based reward model generated with the baseline pipeline in Study 1.}
  \Description{}
  \label{accuracy_diff_s1}
\end{figure}


\subsubsection{S1 -- Comparison to Supervised Learning}

With all 30 training samples, the average balanced accuracy of the individual models ($M^\text{ind}_i$) was 59\% (95\% CI: [53\%, 65\%]) while the collective model ($M^{\text{col}}$) achieved 48\% (95\% CI: [46\%, 50\%]). \autoref{SL_s1} illustrates the relationship between model performance and the number of samples provided per participant.
\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{figures/sl_s1.png}
  \caption{\todo{}}
  \Description{}
  \label{SL_s1}
\end{figure}


\subsection{S1 -- Qualitative Results}
% \todo{put something here}
\subsubsection{S1 -- Qualitative Analysis of Participant Decision Making}\label{section:s1_features}

\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{figures/feature_matrix_s1.png}
  \caption{Behavioural features participants used to decide whether the agent was acting respectfully in Study 1.}
  \Description{}
  \label{respect_features}
\end{figure*}

While our system is designed to align AI agents with a range of user-defined values, our evaluation concentrated on the singular value of respect. Focusing on a single value limited the variability in the study and allowed us to assess the personal and subjective nature of even a single value.

We analyzed the user's conversations with the system in Study 1 to understand what each participant thought respectful behaviour in this environment was. We found 12 behavioural features that participants used to explain whether they thought the agent was respectful. Interestingly, P1 only used one behavioural feature, namely whether the agent stayed in the quadrant it owned, to determine whether the agent acted respectfully. In contrast, P5, P7, and P10 explained whether the agent acted respectfully using seven features. Overall, only one pair of participants used the same features to make their decisions. Further, participants combined the features in diverse ways, such as forming hierarchies of importance or combining them conditionally. The 12 features we identified are:
\begin{enumerate}
    \item \textbf{Stays in Own Quadrant:} Whether the main agent stays in the orchard (quadrant) they own.
    \item \textbf{Interferes With Others:} This feature evaluates a relatively wide range of behaviours, including if the agent appeared to attempt to block another agent, following another agent, or getting too close to another agent.
    \item \textbf{Task Completion:} Whether the agent works toward or completes the task the participant thought the agent should be doing. For example, an agent picking up all apples or garbage in their quadrant. 
    \item \textbf{Picks Up Own Garbage:} Whether the agent picks up garbage in their own orchard (quadrant)
    \item \textbf{Picks Up Others' Garbage:} Whether the agent picks up garbage in other agents orchards
    \item \textbf{Tit for Tat Behaviour: }Some participants explained that a given behaviour was respectful if another agent had done it to them first, such as entering their quadrant.
    \item \textbf{Taking Others' Apples}: Whether the agent picks up apples in orchards it does not own.
    \item \textbf{Eats Own Apples: }Whether the agent eats any apples in their own quadrant.
    \item \textbf{Picks Up Garbage Before Apple:} Whether the agent picks up garbage before eating apples in their own or other quadrants.
    \item \textbf{Efficiency: }Whether the agent moves around without collecting apples or garbage or makes repetitive, futile movements
    \item \textbf{Time in Others' Quadrants:} The duration of time spent in other agents' orchards.
    \item \textbf{In Quadrant While Owner was Gone: }If the agent entered another agent's quadrant while they were gone.
\end{enumerate}

Among the features, the most commonly used was \textbf{Stays in Own Quadrant}, but participants often found other features more important. Some features are temporally static, while others span multiple steps. For example, whether an agent is in its quadrant can be determined at a single time, but whether an agent picked up garbage before eating an apple must be determined over multiple steps. The features each participant used are shown in \autoref{respect_features}.

\subsubsection{S1 -- Analysis of Feature Similarity Between Participants. }

We observed an average Jaccard similarity coefficient between all pairs of participants' feature usage of $J = 0.357$, with a 95\% confidence interval of $(0.333, 0.3813)$

\begin{figure*}
  \centering
  \includegraphics[width=0.5\linewidth]{figures/feature_matrix_S1_jaccard.png}
  \caption{\todo{JACCARD. Put in the appendix?}}
  \Description{}
  \label{jaccard_s1}
\end{figure*}

% \textbf{Evolving Understanding of Respect}.
% A salient finding from our analysis of interview data is the dynamic nature of participants' definitions of respect, which evolved significantly through interaction with the system. This evolution was experience by a broad spectrum of participants (e.g., P19, P10, P7, P18, P20). Initially, many held simplistic conceptions of respect, often tied to the agent remaining within it's own orchard or performing specific tasks such as collecting one's own apples or helping another agent pick up garbage. However, through engaging with the system—particularly via exposure to examples and system feedback—participants' understandings of respect underwent a transformation. This process was further catalyzed by the system's presentation of alternative definitions and hypotheses, prompting deeper reflection and consideration among participants. The shift in perspective was marked, moving from a narrow focus on specific actions to a more nuanced understanding of respect, influenced strongly by the context of interactions and the intentions behind actions.

% \textbf{Evolving Understanding of Respect}.
% A recurrent theme across several participants (e.g., P19, P10, P7) was an initial simplistic definition of respect, often tied to spatial boundaries or specific actions like collecting one's own apples or staying within one's quadrant. For many participants (P19, P18, P10), their definition of respect evolved through interaction with the system. This evolution was prompted by seeing examples, receiving system feedback, and reflecting on alternative definitions presented by the system.

% \textbf{Impact of Examples and Interaction}.
% Interaction with the system and exposure to examples of the agent behaving in various ways played a role in clarifying and refining participants' definitions of respect (e.g., P18, P20). It helped participants articulate their thoughts more clearly and consider behaviours they hadn't initially.
% % Participants P1 and P11 found it hard to label actions that seemed neutral, highlighting the existence of grey areas in defining respectful or disrespectful behaviour.

% \textbf{Role of System Feedback and Hypotheses}.
% The system's hypothesis and the presentation of alternative features also influenced participants' understanding and definition of respect (e.g., P18, P13, P3). It helped some participants narrow down their definitions (P20) or consider aspects they hadn't initially thought of. While the system's alternative definitions helped refine participants' understanding, they did not always change participants' minds about what constitutes respectful behaviour (e.g., P19).

% \textbf{Complexity in Defining Respectful Behavior}.
% Several participants (e.g., P12, P17, P15) faced difficulty in labelling actions as strictly respectful or disrespectful, indicating the complex nature of respect that cannot always be boiled down to binary decisions.
% Participants like P1 and P17 applied specific criteria or logic to decide on what constitutes respect. 


% \textbf{Personalized Definitions and Intuition}.
% The data shows a wide variability in how participants defined respect, with some relying on intuitive understandings that evolved over time (e.g., P6, P4). Participants consistently noted the difficulty in classifying actions that did not clearly align with their definitions of respect, indicating a need for a "neutral" category or more nuanced labelling options.

\subsubsection{S1 -- Thematic Analysis of Interview Data} Through our thematic analysis, we found two main themes: (1) participants' definitions of respect evolved throughout the activity, and (2) The system's hypothesis and alternative perspectives had a specific impact on this evolution.
% Through our thematic analysis, we identified a number of themes, \todo{}
 \space
 
\textit{\textbf{Evolving Definitions of Respect.}}
% \subsubsection*{}
The interview data illustrates that participants' understandings of respect evolved significantly through interaction with the system, particularly influenced by exposure to examples and the system's alternative features. This finding aligns with previous work in consumer research, which found that engaging users in reflection and allowing them to make realistic decisions increases the accuracy of their reported preferences~\cite{hauser2014self}. Initially, many participants held simplistic definitions of respect, often related to spatial boundaries or specific tasks like collecting one's own apples (P4, P6, P7, P10, P19). However, these definitions became more nuanced as participants engaged with the system. The evolution was often spurred by witnessing examples that challenged their initial views and contemplating alternative definitions presented by the system (P3, P8, P10, P13, P18, P19, P20). This highlights a process where the system's feedback and the act of labelling examples prompted participants to refine and sometimes expand their conceptualization of respect, moving beyond their initial assumptions.

\textit{\textbf{Specific Impact of System Hypothesis.}}
% \subsubsection*{Impact of System Hypothesis}
Another recurrent theme was the influence of the system's hypotheses and feedback on shaping participants' conceptions of respect. Participants reported that the system's presentation of alternative features and hypotheses prompted reevaluation, clarification and, in some cases, a significant revision of their definitions of respect (e.g., P3, P8, P13, P18, P20). For instance, the system's suggestions helped participants to narrow down their considerations (P13, P18) or to think about respect in ways they had not initially contemplated (P3, P20). While the system's alternative features did not always change participants' minds (e.g., P19), they played a role in the iterative process of refining participants' understandings, illustrating the value of engaging the user in reflective dialogue.


% \subsubsection*{Complexity in Defining Respectful Behavior}
% The complexity of defining respectful behaviour was a central theme, with some participants expressing difficulty in making a binary  ``respectful'' or ``disrespectful'' categorization of agent behaviour (e.g., P12, P17, P15, P1, P11). Moreover, the existence of grey areas and neutral actions was noted (P1, P11).

% \subsection{Definitions of Respect}\label{definitions_of_respect}

 

% \begin{itemize}
%     \item Multiple participants seemed to want to factor in efficiency or task performance into their definition of respect. I think there may be some implicit understanding that the "right" thing to do in games is get a high score. However, one user said they noticed this about themselves and consciously focused on not letting this determine their respectful labels. Another participant said that since the agent gets reward for picking up apples, this must be a task that the designer wanted the agent to do. Thus reward maximizing while staying in the quadrant is the nice thing to do.
%     \item Multiple users noted that seeing the system's understanding of their definition of respect and also the other factors that could be considered helped them understand their definition. This could be related to the participants asking the researcher what the definition of respect was. It seems as though some participants are not sure about their own definition of a value and need help reflecting. 
%     \item One participant pointed out the agents that did not move. They mentioned that it was difficult to evaluate if the main blue agent was acting disrespectfully when it took their apples because it seemed like they didn't want the apples anyway. 
%     \item One participant noted that if the main agent went into the quadrant owned by an agent that had entered the main agent's quadrant, this was respectful. They mentioned that it was a kind of tit-for-tat. 
%     \item A main theme seems to be that of efficiency vs. respect. Some think they are opposed and some think that they almost mean the same thing, and yet others think that they are not related at all (some said respect was just based on boundaries).
    
% \end{itemize}

\subsection{S1 -- Discussion}\label{section:s1_discussion}
\textit{\textbf{The Diversity of Values (RQ1):}} We developed our system based on the hypothesis that human values and individuals' understandings of human values are diverse. Multiple pieces of evidence point to this being true.


When asked to evaluate whether an agent acted respectfully according to their understanding, participants used vastly different behavioural features to explain whether or not the agent was acting respectfully. We identified 12 behavioural features on which participants based their explanations. All participants, aside from one pair, used a different subset of behavioural features and combined them uniquely. 


Our qualitative results on the diversity of participants' definitions of respect are supported by our analysis of the inter-annotator agreement between the participants when labelling videos as respectful or not. In particular, we only found a ``fair'' agreement between participants ($\kappa = 0.23$). 

The collective reward model's ($M^\text{col}$) performance provides further evidence for the diversity of individual interpretations of respect. Despite having access to 630 samples (21 participants × 30 samples), the collective model's balanced accuracy remained close to random performance whereas the individual models' average balanced accuracy was significantly higher than 50\%. This strongly suggests that participants' labels regarding respectful agent behaviour were sufficiently diverse and potentially contradictory to make it impractical to learn a single, collective definition of respect.



\textit{\textbf{The Importance of Reflection (RQ2):}}
% \subsubsection*{}
When comparing our system to the baseline that does not engage the user in higher-order reflection, we found that our system was significantly more accurate in capturing users' individual definitions of respect. This points to the fact that encouraging the user to consider alternative perspectives and reflect on their preferences allows them to communicate their intent more clearly to the system. 

The qualitative results also support this conclusion. Many participants (P3, P4, P9, P13, P16, P18, P20, P21) noted that seeing and responding to the hypothesis proposed by the system about what features they were using to determine if the agent was acting respectfully and the alternative features, allowed them to either refine, better explain, or clarify their understanding of respectful behaviour.


% \textit{\textbf{The Limitations of Collective Supervised Learning for Subjective Values. }}

\textit{\textbf{Supervised Learning vs. Few-Shot Language-Based Learning (RQ3): }}While individual reward models performed better than the collective approach, even with significantly fewer samples (1/21st of the collective dataset), their average performance was still significantly below \systemname{}. Notably, our system achieved superior results using only four samples per participant compared to the 30 samples used by individual models.

These findings underscore two points: first, the importance of tailoring value alignment to individual perspectives rather than aggregating data, and second, the efficiency of our reflection-based approach in capturing individual value interpretations with minimal data. Our system's ability to achieve higher accuracy with fewer samples highlights the power of structured reflection, iterative refinement, and few-shot language-based learning in eliciting and modelling complex, subjective values.



==> versions/v2.sep.10/6_study2.tex <==
\section{Study 2 - The Moral Machine}
Study 2 investigates the utility of our system for learning about participants' decision-making in moral dilemmas involving an agent (autonomous vehicle). The goal is to understand if our system, which uses reflective dialogue, can effectively capture individual definitions of moral behaviour and whether individual definitions differ. 

\textit{\textbf{Environment \& Task.}}
The Moral Machine dataset \cite{awad2018moral} is based on a simulated environment that presents ethical dilemmas faced by autonomous vehicles. In each scenario, a self-driving car encounters an unavoidable accident and must choose between two outcomes: staying on course or swerving. Each decision results in different consequences for the individuals involved. The environment populates these scenarios with characters chosen from 20 predefined types, including pedestrians, passengers, and various demographic groups such as children, adults, elderly, and animals. Each outcome features between one and five characters.
The scenarios explore nine key ethical dimensions: the nature of the vehicle's intervention, the relationship of individuals to the vehicle (pedestrians or passengers), the legality of pedestrians' actions, and various attributes of potential victims, including age, gender, social status, physical fitness, number, and species (human or pet).

\textit{\textbf{Baselines.}}
In this study, we compared our system to another language-based system described in subsection \ref{baseline} and various reward models trained with supervised learning. Each scenario in the Moral Machine dataset can be represented by a 26-dimension vector that can serve as the input to a model. This representation is easier to learn from than an image representing the scenario, as there is more information per dimension (i.e. there is uninformative information in the image). As such, we try two variations of supervised learning: a multi-layer perception (MLP) from the 26-dimension feature representation and a convolutional neural network (CNN) from the image representation of the scenario. For both the MLP and CNN versions we train two types of reward models: Individual models, $M^\text{ind}$, and a collective model, $M^\text{col}$. 

% One individual model was incrementally trained for each participant, and one collective model was trained for all participants. These models are MLPs with one hidden layer with 32 neurons, trained with a learning rate of $0.001$ and the Adam optimizer. The input to the models was the numerical encoding shown in \autoref{numerical_encoding}.

\textit{\textbf{Participants.}}
% \subsubsection*{Participants}
We recruited 9 participants from our institution (18 to 33 age range, M=25.66, 6 self-identified as male and 3 as female). When asked to rate their level of familiarity with reinforcement learning on a 5-point Likert ranging from ``very unfamiliar'' (1) to ``very familiar'' (5), the mean level of familiarity was 3.55, with the mode and median being 3. The Likert-scale data is visualized in figure \ref{fig:rl_familiar_s2}.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.5\linewidth]{figures/rl_familiar_S2.png}
  \caption{Participant familiarity with reinforcement learning in Study 1.}
  \Description{}
  \label{fig:rl_familiar_s2}
\end{figure}

% \textit{\textbf{Grid World Environment: }}






% To answer the second question, we measure how much the reward models produced by each pipeline agree with the participants they are modelling. We then compare this to how much the participants agree with one another. Specifically, we created two reward models for each participant: one using the baseline pipeline and another using our pipeline (as described in section \ref{partic_reward_modelling}). We assess the agreement between each participant's responses and their corresponding reward models using the Fleiss' kappa metric. By averaging these agreement scores across all participants for both pipelines, we obtain a measure of how well the reward models from each pipeline match the participants' views. We also bootstrap the agreement scores to obtain confidence intervals for the average agreement between the participants and the reward models from each pipeline. We then calculate the inter-annotator agreement between all participants again using Fleiss' kappa. \todo{add citation and explanation for the choice of Fleiss' kappa. Maybe add a word of warning?}

\subsection{S2 -- Quantitative Results}

On average, participants took 18 minutes 28 seconds (SD $=$ 7 min. 15 sec., range: 12 min. 0 sec. - 34 min. 34 sec.) to complete the dialogue with the system and 11 minutes 51 seconds (SD $=$ 4 min. 15 sec., range: 4 min. 46 sec. - 17 min. 04 sec.) to complete the labelling of 50 trajectories. Of 9 participants, 1 (11.$\bar{11}\%$) entered the \textit{preference clarification loop} for one iteration.

\subsubsection{S2 - Inter-Annotator Agreement}
We observed a Fleiss' kappa value between all participants' labels on the 50 labelled trajectories of $\kappa = 0.460$, indicating ``moderate'' (higher than ``fair'') agreement among participants \cite{landis1977measurement}.

\subsubsection{S2 -- Evaluation of Language-Based Reward Model Performance.}
On average, the reward models produced by our pipeline received significantly higher accuracy scores (measured in percentages) than the baseline system by 12\% (95\% CI: [4\%, 27\%], M = $65\%$ vs. M = $53\%$, p=.05). The distributions of the balanced accuracies for each pipeline are visualized in \autoref{accuracy_dist_S2}. The distribution of the per participant difference in balanced accuracy is shown in \autoref{accuracy_diff_S2}



% The average Fleiss' kappa statistic for the reward models generated with the baseline system and the participants was $\kappa = 0.25$ (95\% CI:[0.14, 0.35]), indicating. The average Fleiss' kappa for the reward models generated with our pipeline and the participants was $\kappa = 0.36$ (95\% CI:[0.28, 0.43]).

% This result indicates that the reward models produced by our pipeline, using \systemname{}, on average, agree more with each participant than the participants agree with each other about what agent behaviour is respectful. \carter{However, this result should be taken with caution?}

\begin{figure}
  \centering
  \includegraphics[width=0.5\linewidth]{figures/accuracy_comparison_S2.png}
  \caption{Distributions of the accuracies of the language-based reward models generated with our pipeline (IRDA) compared to those of the language-based reward model generated with the baseline pipeline in Study 2.}
  \Description{}
  \label{accuracy_dist_S2}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=0.5\linewidth]{figures/accuracy_diff_S2.png}
  \caption{Distribution of the per participant difference in accuracy between the language-based reward model generated with our pipeline (IRDA) compared to the language-based reward model generated with the baseline pipeline in Study 2.}
  \Description{}
  \label{accuracy_diff_S2}
\end{figure}

\subsubsection{S2 -- Comparison to Supervised Learning}
In this study, we trained two types of reward models with supervised learning: a simple MLP and a Convolutional Neural Network. \todo{redundant} One version is based on a simple MLP network with one hidden layer of 32 neurons and uses a highly processed (feature-engineered) input. The other is a convolutional neural network (CNN) \todo{Put details in appendix} consisting of two convolutional layers, each followed by a Rectified Linear Unit (ReLU) activation function and max pooling operation. These initial layers are responsible for extracting and refining visual features from the input images. Following the convolutional layers, the network uses a flattening operation to convert the 2D feature maps into a 1D vector. This flattened representation is then fed into a fully connected layer with ReLU activation, which further processes the extracted features. The network culminates in a final output layer with two neurons, corresponding to the two classes in the binary classification task. 


The Moral Machine setting lends itself to an easy \todo{featurization} (i.e., the scenarios can be succinctly described numerically), and we trained the MLP on this. For the CNN, we used images of the moral machine scenarios. Since the CNN must learn the relevant features in the convolutional layers, as opposed to being provided them, the learning problem is more difficult. 

With all 30 training samples, the average accuracy of the individual MLP models ($M^\text{ind}_i$ (MLP)) was 79\% (95\% CI: [74\%, 83\%]) while the collective model ($M^{\text{col}}$ (MLP)) achieved 79\% (95\% CI: [77\%, 81\%]). \autoref{SL_S2} illustrates the relationship between model performance and the number of samples provided per participant for the MLP models.
\begin{figure}
  \centering
\includegraphics[width=0.5\textwidth]{figures/sl_S2.png}
  \caption{\todo{}}
  \Description{}
  \label{SL_S2}
\end{figure}

For the CNN models, with all 30 training samples, the average accuracy of the individual models ($M^\text{ind}_i$ (CNN)) was 67\% (95\% CI: [61\%, 73\%]) while the collective model ($M^{\text{col}}$ (CNN)) achieved 77\% (95\% CI: [70\%, 83\%]). \autoref{SL_S2_cv_CNN} illustrates the relationship between model performance and the number of samples provided per participant for the CNN models.

\begin{figure}
  \centering
\includegraphics[width=0.5\textwidth]{figures/sl_S2_cv_CNN.png}
  \caption{\todo{}}
  \Description{}
  \label{SL_S2_cv_CNN}
\end{figure}


\subsection{S2 -- Qualitative Results}

\subsubsection{S2 -- Qualitative Analysis of Participant Decision Making}\label{section:s2_features}

\begin{figure*}
  \centering
  \includegraphics[width=0.5\linewidth]{figures/feature_matrix_S2.png}
  \caption{Behavioural features participants used to decide what the autonomous vehicle should do in Study 2.}
  \Description{}
  \label{features_S2}
\end{figure*}

By analyzing the participants' conversations with our system, we identified nine features they used in their decision-making in Study 2. The features we identified are:
\begin{enumerate}
    \item \textbf{Human vs. Animal Priority:} Whether human lives are prioritized over animal lives.
    \item \textbf{Traffic Rule Compliance:} The consideration of the legality of pedestrians' actions.
    \item \textbf{Minimizing Casualties:} The aim to minimize the total number of fatalities.
    \item \textbf{Age Prioritization:} The preference for saving younger people over older people.
    \item \textbf{Survival Probability:} The consideration of the likelihood of survival for different individuals based on factors like physical fitness.
    \item \textbf{Maintaining Original Path:} The preference for the vehicle to stay on its original course rather than swerving.
    \item \textbf{Societal Value:} The consideration of perceived societal value or potential future contributions of individuals.
    \item \textbf{Passenger Safety Priority:} The prioritization of the safety of the vehicle's passengers over pedestrians or other road users.
    \item \textbf{Gender:} The consideration of the gender of potential victims in the decision-making process.
\end{enumerate}

Like Study 1, participants combined and used these features in various ways.

\subsubsection{S2 -- Analysis of Feature Similarity Between Participants. }

We observed an average Jaccard similarity coefficient between all pairs of participants' feature usage of $J = 0.464$, with a 95\% confidence interval of $(0.403, 0.526)$

\begin{figure*}
  \centering
  \includegraphics[width=0.5\linewidth]{figures/feature_matrix_S2_jaccard.png}
  \caption{\todo{}}
  \Description{}
  \label{jaccard_s1}
\end{figure*}

\subsubsection{S2 -- Thematic Analysis of Interview Data}

\textit{\textbf{Decision-making Evolution. }}
Our results reveal a divergence in how participants' decision-making processes evolved throughout the study. Some participants reported that their approach changed as they encountered a wider range of scenarios. For instance, P3 noted that "as more cases came up, I realized the need to consider new factors when the initial factors were equal between groups." This reiterates our finding from Study 1 that exposure to diverse situations can prompt users to refine and expand their decision-making criteria. Conversely, other participants maintained consistent rules throughout the study. P2 stated that their "rules remained consistent throughout," indicating that some users may approach such tasks with pre-established ethical frameworks that remain stable across various scenarios. 
% This divergence highlights the importance of considering individual differences in ethical reasoning when designing AI systems that involve human-in-the-loop decision making.

% \textit{\textbf{Impact of AI Feedback. }}
% Compared to Study 1, participants were less influenced by the reflective dialogue offered by the system. While P5 reported changing their answers based on the reflective dialogue offered by the system and entered the preference clarification loop, no other participants entered the preference clarification loop.

\textit{\textbf{Intuition vs. Explicit Reasoning. }}
Our findings reveal an interplay between explicit reasoning and intuition. Most participants felt capable of articulating their decision-making process. Still, the emergence of intuition-based decisions in particularly challenging scenarios, as reported by P6 and P7, underscores the complexity of ethical reasoning. P7 mentioned relying on "first instinct" or "vibes" for 3 or 4 especially difficult scenarios. 
% This finding has important implications for the design of ethical AI systems. While promoting explicit reasoning is generally desirable, interfaces should also acknowledge and potentially accommodate intuitive decision-making in complex cases. Future research could explore how to balance these two modes of thinking in AI-assisted ethical decision-making tools.
% Value of Scenario Exposure
% The study underscores the importance of exposing users to a diverse range of scenarios when engaging with ethical decision-making systems. Several participants, including P3 and P4, emphasized that encountering different scenarios helped them develop or refine their decision-making process. This suggests that scenario-based learning could be an effective approach for training users to interact with AI systems that handle ethical dilemmas.

% \textit{\textbf{Comprehensiveness of Explanations. }}
% Most participants felt that their explanations during the dialogue phase captured a significant portion (90\% or more) of their decision-making process. This finding, reported by P6 and P7, suggests that the dialogue-based approach was largely successful in eliciting comprehensive explanations from users.

\subsection{S2 -- Discussion}

\textit{\textbf{Reflection and Preference Communication (RQ2):}}
Unlike in Study 1, participants in this study exhibited more fixed opinions, with fewer entering the preference 
clarification loop. This highlights an important aspect of our system: the value of reflection extends beyond clarifying users' thoughts; it is a powerful tool for effective preference communication. When the system presents alternative perspectives, users need not adopt these viewpoints. Instead, engaging with these alternatives and articulating their stance improves the system's understanding of their preferences. This structured reflection process allows users to more precisely convey their decision-making rationale, even if their fundamental views remain unchanged. Notably, despite the reduced engagement with the clarification loop, our system still outperformed the language-based reward modelling baseline. This underscores the efficacy of our approach in preference elicitation, demonstrating that even limited interaction with diverse viewpoints can significantly enhance the system's understanding of user preferences. 

\textit{\textbf{Sample Efficiency vs. Traditional Methods (RQ3):}}
Our analysis of supervised learning approaches revealed that with sufficient samples, traditional methods can 
surpass our system's performance, particularly when using feature-engineered inputs (MLP model) as shown in \autoref{SL_S2}. The collective MLP model's ($M^{\text{col}}$) performance increased rapidly, while individual models ($M^{\text{ind}}$) improved more slowly due to fewer samples per participant. With around 15 samples per participant, individual models also surpassed our system. However, our method remains the most sample-efficient, achieving comparable performance with just four samples.

\textit{\textbf{The Impact of Input Representation (RQ3): }}
The difference in performance between the MLP (using feature-engineered inputs) and CNN (using image 
inputs) models highlights the importance of input representation in learning users' preferences. This disparity suggests that explicit feature identification, a core aspect of our dialogue-based approach, is crucial in efficiently capturing users' decision-making processes.

\textit{\textbf{Context-Dependent Effectiveness (RQ3):}}
Our findings indicate that the effectiveness of reward modelling methods is context-dependent. Traditional reward modelling methods may be more effective given sufficient samples in scenarios with high inter-annotator agreement and easily learnable features. Conversely, our few-shot language-based approach performs favourably in more complex scenarios with low agreement and when sample efficiency is crucial.

==> versions/v2.sep.10/7_discussion.tex <==
\section{Discussion}

Here, we discuss and reflect on important findings from the development and evaluations of \systemname{}; we note limitations and opportunities for future work. 

% \subsubsection*{Generation vs. Evaluation}
% Previous work on using natural language reward models by Kwon et al.~\cite{kwon2022reward} prompted users to come up with examples of the behaviour they would like the agent to embody. While this gives the user a high degree of control, we overwhelmingly found that participants did not initially know what behaviours they thought were respectful. Participants mentioned that seeing various trajectories of the agent behaving in the environment allowed them to understand better what they thought was respectful. Further, participants found that the system's hypothesis and proposition of alternative features were useful for framing and clarifying their thinking.

% In sum, our results indicate that giving the user examples to evaluate will likely lead to more accurate reward models than having the user generate examples on their own.

\subsection{Key Findings and Implications}

\subsubsection{Heterogeneity of Opinions and Model Performance}
Study 2 demonstrated more homogeneous opinions compared to Study 1, as evidenced by higher inter-annotator 
agreement ($\kappa$ = 0.460 vs $\kappa$ = 0.336) and greater feature usage similarity ($J = 0.464$ vs $J = 0.357$). This homogeneity allowed collective models to perform well in Study 2, whereas in Study 1, the collective model struggled despite the size of the training set. This underscores the challenge of developing universal value-aligned AI systems and highlights the need for more representative reward modelling approaches in domains with diverse individual preferences.

\subsubsection{Non-Markovian Behavioural Features}

In Study 1, we found that some of the features used by participants to determine whether the agent's behaviour was respectful violate the Markov property. This means the behavioural feature could not be assessed in a single time step. An example of a feature that \textit{does} satisfy the Markov property is whether the agent is in its own orchard - the current state holds all the information necessary to determine the feature. An example of a behavioural feature that \textit{violates} the Markov property is whether or not the agent picked up garbage \textit{before} collecting an apple. This feature requires information from at least two time steps to be determined. Similarly, some participants considered whether an agent went into the quadrant of another agent that had already been in their quadrant.

Since some of the features participants used are non-Markovian, it is important to have a reward model that can capture this. If, for example, the reward model only receives a single step as input (as is common in traditional RL), these non-Markovian features cannot be captured. The reward models produced by our pipeline take an entire trajectory as input. While this can be less precise, it allows for using non-Markovian features to determine the reward. 

\subsubsection{Efficacy of Few-Shot Language-Based Reward Modeling}
When the sample size is limited, or when there's low agreement among users, and the learning problem is complex, few-shot language-based reward modelling with structured reflection was most effective. Our system outperforms traditional supervised learning methods in these scenarios, offering a viable solution for real-world applications where extensive data collection is impractical or where preferences are highly individualized. 

\subsubsection{Dual Benefits of Reflection}
The reflection process in our system serves two crucial functions: it helps users clarify their own 
understanding of their preferences, and it enables more effective communication of these preferences to the 
system. Even when users' opinions remain unchanged, engaging with alternative perspectives enhances the 
system's ability to capture nuanced preferences accurately.


\subsubsection{Democratization}
In some cases, people may want to train agents to align with their individual values and preferences. For example, users may want AI systems in their home to align with their values. As such, there is a need for accessible solutions to align agents with individual values. In our study, a majority of the participants were either ``very unfamiliar'' or ``unfamiliar'' with reinforcement learning. Yet, the system was still able to capture their definition of respect, allowing them to create a reward model that could be used to train an agent. 

 \subsection{Ethical Considerations}
 While the personalization of AI systems and agents has advantages, there are also risks. Due to the inherent diversity of values and preferences, sometimes aligning to one person's definition of a value means unaligning from others'. For example, if one person believes that it is respectful for their agent to pick up garbage on their neighbour's property, but the neighbour does not believe this is respectful, we reach a conflict. In cases such as this, where multiple stakeholders will be impacted, using the individualized reward models as proxies for the stakeholders and making a fair trade-off is more suitable.

Further, while we exemplified the use of our system, \systemname{}, for aligning agents to respectful behaviour, we acknowledge that the system could be used to train agents with more nefarious values. Because of this, before deploying a system for personalizing AI agents, it is important to build guard rails that limit the range of possible behaviours that can be trained into the agent. While this is important, the focus of our paper is not building guardrails, and this is better left for other, more dedicated treatments. 

\subsection{Limitations}

\subsubsection{Implementation Dependence}

Some aspects of our system are artifacts resulting from the current capabilities of large language and vision language models. For example, we textually encode trajectories so that they can be input into a language model. We chose this because vision language models performed poorly in the environments we tested. However, this may not be necessary in the future as the capabilities of LLMs and VLMs increase. That said, the core of the system, namely the overall pipeline, is not model dependent, and as capabilities increase, we expect the performance of the pipeline only to increase. 

\subsubsection{Reward Model vs. Agent Accuracy}
We focused our system and evaluation on the feedback collection and reward modelling phases of the RLHF pipeline and did not consider policy optimization (agent training). We chose this because our core innovation is not related to policy optimization. This leaves questions open about the behaviour that would result from training an agent with a reward model produced by our system. However, Kwon et al. \cite{kwon2022reward} found that RL agent accuracy mimics the reward model accuracy.

% \subsubsection*{Binary Labels}
%  Multiple participants mentioned that it was difficult to classify some trajectories as either respectful or disrespectful and that some seemed neutral. As such, the fact that our system uses binary reward could be seen as a drawback. 
%  % In RLHF it is common to use pairwise comparisons where participants would, for example, decide which of two options is ``more respectful.''
 
% \subsubsection*{Environment Complexity}
% The environment we used to evaluate our system is relatively simple and abstract. Using our system in more realistic environments could present new challenges, but it could also be easier in some ways. For example, perhaps vision language models would perform well in more realistic environments.

\subsection{Future Work}
There are likely many possible interface improvements that would make the system more usable and accessible, as well as algorithmic improvements that would make our system more performant. We believe discovering and developing these improvements is an exciting line of research. 

% \subsubsection*{Pipeline Improvements}
% LLMs are expensive

\subsubsection{Interactive RLHF}
In our studies, we looked specifically into reward modelling and did not train agents with the reward models generated by our system. However, each type of reward model, including the ones generated by our system and the ones we compared to, had imperfections. These imperfections can result in imperfect agents. As such, future work can examine how to interleave reward modelling and agent training. In this way, the user can iteratively give feedback directly addressing the trained agent's imperfections. 

\subsubsection{Aligning to Group vs. Individual Values}
Our work has focused on learning reward models that mimic an individual. While this approach can be used for personalization, it can be extended to group alignment by considering the group's preferences as an aggregation of its members' individual preferences. While this method has been previously explored in the context of collective decision-making and virtual democracy \cite{noothigattu2018voting, freedman2020adapting, mohsin2021making, gordon2022jury}, applying it to align an agent's behaviour with a group's preferences is a promising avenue for future research.

% \subsubsection*{Integration of Pairwise Comparisons}
% Pairwise comparisons can be useful for eliciting preferences as they allow annotators to make relative assessments instead of absolute assessments. Integrating pairwise comparisons into our system's dialogue-based preference elicitation phase could help address the difficulty some participants had in deciding between binary labels.

% \subsubsection*{More Values in More Realistic Environments}
% We evaluated the efficacy of our system in capturing individual users' definitions of respect in a multi-agent grid world environment. Future work could adapt the system to more realistic environments. It could be the case that VLMs work more effectively in more complex environments as the data is likely closer to the distribution of the training data.
 


==> versions/v2.sep.10/8_conclusion.tex <==
\section{Conclusion}

We developed a system, \systemname{}, that allows users with no particular experience in machine learning to train agent's in alignment with their individual understanding of values. In a user study where participants evaluated whether an agent's behaviour was respectful or not, we found that different people have vastly different definitions of what respectful behaviour is. Further, we found that our system was able to capture each individual's definition of such behaviour to a relatively high degree of accuracy.
